HS-Pose: Hybrid Scope Feature Extraction for Category-level Object Pose Estimation

In this paper, we focus on the problem of category-level object pose estimation, which is challenging due to the large intra-category shape variation. 3D graph convolution (3D-GC) based methods have been widely used to extract local geometric features, but they have limitations for complex shaped objects and are sensitive to noise. Moreover, the scale and translation invariant properties of 3D-GC restrict the perception of an object's size and translation information. In this paper, we propose a simple network structure, the HS-layer, which extends 3D-GC to extract hybrid scope latent features from point cloud data for category-level object pose estimation tasks. The proposed HS-layer: 1) is able to perceive local-global geometric structure and global information, 2) is robust to noise, and 3) can encode size and translation information. Our experiments show that the simple replacement of the 3D-GC layer with the proposed HS-layer on the baseline method (GPV-Pose) achieves a significant improvement, with the performance increased by 14.5% on 5d2cm metric and 10.3% on IoU75. Our method outperforms the state-of-the-art methods by a large margin (8.3% on 5d2cm, 6.9% on IoU75) on the REAL275 dataset and runs in real-time (50 FPS).

==> CVPR2023/fig/3dgcn_structure/item.tex <==
\begin{figure}
% \vspace{-1mm}
\centering
\vspace{-5mm}
\includegraphics[width=0.5\linewidth]{CVPR2023/fig/3dgcn_structure/inner_structure.pdf}
\vspace{-8mm}
\caption{\footnotesize \textbf{The inner structure of the 3D-GC layer.} The input point cloud along with their features are first grouped to receptive fields by RF-P and then passed through the deformable kernel based graph convolution layer. RF-P ensures the feature extraction of local geometry.}
\label{fig:gcn3d}
\vspace{-15px}
\end{figure}             

==> CVPR2023/fig/gpv_pose_framework/item.tex <==
\begin{figure}[ht]
\centering
\vspace{-3mm}
\includegraphics[width=1.0\linewidth, trim = 0 0 0 40 , clip]{CVPR2023/fig/gpv_pose_framework/gpv-pose.jpg}
\vspace{-8mm}
\caption{\textbf{The overall structure of GPV-Pose}.
} 
\vspace{-3mm}
\label{fig:gpv_framework}
\end{figure} 

==> CVPR2023/fig/orl_comp/item.tex <==
\begin{figure}[]
\centering
% \vspace{-1mm}
\includegraphics[width=1\linewidth, trim = 0 20 20 20, clip]{CVPR2023/fig/orl_comp/orl_comp.pdf}
\vspace{-7mm}

\vspace{-1mm}

\end{figure} 


==> CVPR2023/others/other_infos.tex <==
\input{CVPR2023/others/tbl/complete_ablation.tex}
\input{CVPR2023/others/tbl/camera_results.tex}

==> CVPR2023/others/tbl/camera_results.tex <==
\begin{table*}[ht]
\begin{center}

\caption{\textbf{Compare with GPV-Pose on CAMERA dataset.} }
\label{tbl:gpv_cae_camera}

\resizebox{0.8\linewidth}{!}
{%
\footnotesize
\begin{tabularx}{\linewidth}{p{4.2cm}|p{0.9cm}<{\centering}|p{0.5cm}<{\centering}p{0.5cm}<{\centering}p{0.7cm}<{\centering}|p{0.6cm}<{\centering}p{0.6cm}<{\centering}p{0.7cm}<{\centering}p{1.0cm}<{\centering}|p{0.7cm}<{\centering}p{0.7cm}<{\centering}|p{1cm}<{\centering}}
\toprule 
\renewcommand{\multirowsetup}{\centering}%
Method & Type &$\text{IoU}_{25}$   &$\text{IoU}_{50}$    &$\text{IoU}_{75}$     &$5^\circ 2cm$ &$5^\circ 5cm$ &$10^\circ 2cm$ &$10^\circ 5cm$ &$2cm$& $5^\circ$ &Speed(FPS)  \\
\midrule            
\midrule            
% Method|IoU25|IoU50|IoU75|5d2cm|5d5cm|10d2cm| 10d5cm|2cm| 5deg|speed
%----------------------------
GPV-Pose\cite{GPV-Pose_2022_CVPR}(reported) &D & - &93.4 &88.3 &72.1 &80.1 &89.0 &- &- &- & 20\\
GPV-Pose(\textbf{trained by us}) &D &\textbf{95.1} &{92.6} &84.1 &59.4 &69.7 &70.3 &84.6 &- &- &{27}\\

%-----------------------------------
\midrule
\textbf{Ours} (GPV-Pose+CAE)  &D &\textbf{95.0} &92.7 &\textbf{87.6} & \textbf{69.0} &\textbf{77.5} &\textbf{76.7} & \textbf{87.6} &\textbf{89.3} & \textbf{78.8} &20\footnote{Tested on a single RTX3090ti.}\\ 

\bottomrule
\end{tabularx}%
}
\end{center}
\end{table*}

==> CVPR2023/tbl/ablation/ablation.tex <==

% {\small
\begin{table}[ht]
\begin{center}
\caption{\textbf{Ablation studies on REAL275.}}
\label{tbl:ablation}
\vspace{-3mm}
\resizebox{1.0\linewidth}{!}
{
\begin{tabular}{@{}c|l|c|cc|c|c|c@{}}
\toprule

Row    & Comparison   &$\text{IoU}_{75}$ &$5^\circ 2\text{cm}$ &$5^\circ 5\text{cm}$ &$5^\circ$ &$2\text{cm}$ & speed\\
\midrule
\midrule            
% %
A0 & \textbf{Ours} (B0+STL+FPG+LGL) &\underline{74.5} & \textbf{46.1} &\textbf{55.2} & \underline{58.3} & \textbf{78.1} \\
\hline
B0 &GPV-Pose(baseline) &64.4 &32.0 &42.9 & 44.7 & 69.7 \\
\hline
% C0 &B0: 3DGCN $\rightarrow$ CAE &70.1 &41.9 &49.1 & 52.7& 78.8 \\
C0 &B0 + STL & 73.1 & 36.4 & 45.1 & 47.4& 75.6\\
C1 &B0 + FPG & 67.7 & 38.9 & 52.3 & 56.1 & 71.7\\
C2 &B0 + STL + FPG &{72.0} & {42.7} &{53.7} &{57.0}  &75.7 \\ %&36/42\\ 
% C3 &B0 + STL + FPG + LGL &\underline{74.5} & \textbf{46.1} &\textbf{55.2} & \underline{58.3} & \textbf{78.1} \\
% \hline
% D2 & D0 + FPG &{72.0} & {42.7} &{53.7} &{57.0}  &75.7 \\ %&36/42\\ 
\hline
D0 & A0: LGL $\rightarrow$ mean pool& {73.4} & {43.7} &\underline{54.8} &\textbf{58.5} &75.7\\ 
D1 & A0: LGL $\rightarrow$ max pool& \textbf{74.8} & \underline{44.3} &{54.5} &{58.1} &\underline{77.3}\\ %&49/()
% \hline
% E1 &B0: 3DGCN to PointNet &66.8 &30.4 &36.1 & 39.3& 74.5\\

\bottomrule
\end{tabular}
}
\end{center}
\end{table}
% }


==> CVPR2023/tbl/neighbor_num/ORL_RFF_full.tex <==
\begin{table*}
\begin{center}

\caption{\textbf{Ablation studies on the neighbor number of ORL and RF-F.} }
\vspace{-4mm}
\caption*{\footnotesize Higher score means better performance. Overall best results are in bold, and the second-best results are underlined.}
\label{tbl:ablation_full}
\vspace{-3mm}
\resizebox{0.9\linewidth}{!}
{\footnotesize

\begin{tabular}{@{}c|l|ccc|cccc|cc|c@{}}
\toprule

Row & N_num &$\text{IoU}_{25}$   &$\text{IoU}_{50}$    &$\text{IoU}_{75}$     &$5^\circ 2$cm &$5^\circ 5$cm &$10^\circ 2$cm &$10^\circ 5$cm &$2$cm& $5^\circ$ &Speed(FPS)  \\
\midrule            
\midrule            
% N_num|IoU25|IoU50|IoU75|5d2cm|5d5cm|10d2cm| 10d5cm|2cm| 5deg|speed
%----------------------------
A0 & 3  &84.1 &81.5 &73.1 &39.0 &47.6 &63.5 &76.9 &76.7 &50.7 & 64\\
%-----------------------------------
\midrule
B0 & 5  &84.0 &81.2 &72.7 &41.7 &52.8 &62.4 &78.3 &75.4 &56.0 & 59\\ 

D0 & 10 &84.2 &82.1 &74.7 &46.5 &55.2 &68.6 &82.7 &78.2 &58.2 &50\\ 
 
B1  &20 &84.3 &82.8 &75.3 &46.2 &56.1 &68.9 &84.1 &77.8 &59.1 &38\\ 

B2 & 30 &84.3 &82.3 &75.2 &46.4 &56.6 &68.5 &83.8 &77.0 &59.9 &30\\ 

C0 & 40 &84.3 &8.8 &70.3 &39.6 &55.8 &62.1 &84.3 &70.5 &58.9 &26\\ 

\midrule




\bottomrule
\end{tabular}
}
\vspace{-7mm}
\end{center}
\end{table*}

==> CVPR2023/tbl/neighbor_num/ORL_full.tex <==
\begin{table*}
\begin{center}

\caption{\textbf{Ablation studies on the neighbor number of ORL.} }
\vspace{-4mm}
\caption*{\footnotesize Higher score means better performance. Overall best results are in bold, and the second-best results are underlined.}
\label{tbl:ablation_full}
\vspace{-3mm}
\resizebox{0.9\linewidth}{!}
{\footnotesize

\begin{tabular}{@{}c|l|ccc|cccc|cc|c@{}}
\toprule

Row & N_num &$\text{IoU}_{25}$   &$\text{IoU}_{50}$    &$\text{IoU}_{75}$     &$5^\circ 2$cm &$5^\circ 5$cm &$10^\circ 2$cm &$10^\circ 5$cm &$2$cm& $5^\circ$ &Speed(FPS)  \\
\midrule            
\midrule            
% N_num|IoU25|IoU50|IoU75|5d2cm|5d5cm|10d2cm| 10d5cm|2cm| 5deg|speed
%----------------------------
A0 & 3  &84.3 &82.6 &74.6 &43.3 &53.1 &67.0 &81.6 &77.2 &56.8 & 52\\
%-----------------------------------
\midrule
B0 & 5  &84.1 &82.7 &72.8 &43.6 &53.0 &66.5 &81.3 &76.9 &56.4 & 51\\ 

D0 & 10 &84.2 &82.1 &74.7 &46.5 &55.2 &68.6 &82.7 &78.2 &58.2 &50\\ 

B1 & 20 &84.2 &81.9 &72.7 &42.7 &55.3 &65.3 &82.7 &74.8 &59.1 &48\\ 

B2 & 30 &84.2 &83.0 &73.9 &43.1 &54.4 &67.0 &83.4 &76.6 &57.4 &48\\ 

C0 & 40 &84.2 &83.2 &71.1 &39.4 &53.7 &62.5 &82.5 &71.9 &57.4 &49\\ 

\midrule




\bottomrule
\end{tabular}
}
\vspace{-7mm}
\end{center}
\end{table*}

==> CVPR2023/tbl/neighbor_num/RF-F_full.tex <==
\begin{table*}
\begin{center}

\caption{\textbf{Ablation studies on the neighbor number of RF-F.} }
\vspace{-4mm}
\caption*{\footnotesize Higher score means better performance. Overall best results are in bold, and the second-best results are underlined.}
\label{tbl:RFF_neighbor_all}
\vspace{-3mm}
\resizebox{0.9\linewidth}{!}
{\footnotesize

\begin{tabular}{@{}c|l|ccc|cccc|cc|c@{}}
\toprule

Row & N_num &$\text{IoU}_{25}$   &$\text{IoU}_{50}$    &$\text{IoU}_{75}$     &$5^\circ 2$cm &$5^\circ 5$cm &$10^\circ 2$cm &$10^\circ 5$cm &$2$cm& $5^\circ$ &Speed(FPS)  \\
\midrule            
\midrule            
% N_num|IoU25|IoU50|IoU75|5d2cm|5d5cm|10d2cm|10d5cm|2cm| 5deg|speed
%----------------------------
% Result path: chenwang /output/models/RFF_neighbor_number_test/n_num_03/eval_149_speed/log_eval.txt
A0 & 3  &84.2 &83.1 &72.9 &39.8 &49.2 &64.1 &78.3 &77.5 &52.9 & 64\\ 

%Result path: amax /output/models/RFF_neighbor_number_test/n_num_05/log_eval.txt
B0 & 5  &84.1 &82.4 &72.8 &41.5 &51.4 &63.6 &79.1 &75.6 &55.2 & 60\\ 

D0 & 10 &84.2 &82.1 &74.7 &46.5 &55.2 &68.6 &82.7 &78.2 &58.2 &50\\ 

%Result path: amax /output/models/RFF_neighbor_number_test/n_num_20/eval_149/log_eval.txt
B1 & 20 &84.2 &82.5 &73.4 &46.1 &56.7 &67.7 &83.8 &76.2 &59.6 &41\\ 

%Result path:amax output/models/RFF_neighbor_number_test/n_num_30/log_eval.txt
B2 & 30 &84.3 &82.9 &75.2 &45.2 &55.1 &67.6 &82.9 &76.4 &58.0 &34\\ 

C0 & 40 &84.3 &82.6 &71.9 &41.6 &54.4 &65.7 &85.0 &73.4 &57.5 &30\\ 


\bottomrule
\end{tabular}
}
\vspace{-7mm}
\end{center}
\end{table*}

==> CVPR2023/tbl/quantitative/linemod.tex <==
\begin{table}
\begin{center}

\caption{\textbf{Performance Comparison on the LineMOD Dataset.} }
% \vspace{-4mm}
% \caption*{\footnotesize Higher score means better performance. Overall best results are in bold, and the second-best results are underlined.}
\label{tbl:linemod}
\vspace{-3mm}
\resizebox{0.9\linewidth}{!}
{\footnotesize

\begin{tabular}{@{}c|c|c|c@{}}
\toprule

Method             & Category & ADD(-S) & Speed(FPS)  \\
\midrule            
\midrule            
% N_num|IoU25|IoU50|IoU75|5d2cm|5d5cm|10d2cm| 10d5cm|2cm| 5deg|speed
%----------------------------
% CDPN~\cite{CDPN} &   & 89.86\\
PVNet~\cite{PVNet} &          &86.3 &25 \\
Epro-PnP~\cite{Epro-PnP_2022_CVPR} & & 95.8 &\\
G2L-Net~\cite{G2L_Net} &      &98.7 &23 \\
DenseFusion~\cite{Densefusion_Wang_2019_CVPR} &      &94.3 &16 \\
PVN3D~\cite{PVN3D_CVPR_2019} &      &99.4 &5 \\
%-----------------------------------
\midrule
DualPoseNet~\cite{DualPoseNet_2021_ICCV} &  \checkmark   &98.2 &2 \\
FS-Net~\cite{FSNET_2021_CVPR} & \checkmark   &97.6 &20 \\
GPV-Pose~\cite{GPV-Pose_2022_CVPR} & \checkmark &98.2 &20 \\
\midrule
\textbf{Ours}          &  \checkmark&- & - \\
\bottomrule
\end{tabular}
}
\vspace{-7mm}
\end{center}
\end{table}

%%% 139 epochs
% objects  ape    benchvise  camera  can     cat     driller  duck   eggbox  glue   holepuncher  iron   lamp    phone  Avg(13)
% ad_2     6.67   24.64      10.59   34.15   27.94   37.17    6.85   75.96   74.13  12.84        40.14  58.83   24.36  33.41
% ad_5     71.33  84.48      79.12   92.03   93.61   89.99    70.42  98.69   96.33  83.16        92.65  96.07   87.91  87.37
% ad_10    95.52  95.83      98.43   99.21   99.40   98.02    96.81  99.72   98.17  97.72        97.85  98.85   95.75  97.79
% rete_2   11.62  18.04      16.27   33.76   21.06   35.98    16.62  24.23   15.93  23.88        27.68  32.25   26.44  23.37
% rete_5   63.14  80.80      79.41   87.20   83.73   90.39    70.14  76.90   67.86  79.64        87.74  90.88   79.98  79.83
% rete_10  91.81  97.48      97.45   98.52   98.20   98.71    95.59  93.52   89.58  97.72        98.06  98.94   95.28  96.22
% re_2     11.62  18.23      16.27   33.76   21.06   35.98    16.62  24.23   15.93  23.98        27.78  32.44   26.44  23.41
% re_5     63.14  80.80      79.41   87.20   83.73   90.39    70.14  76.90   67.86  79.64        87.74  90.88   79.98  79.83
% re_10    91.81  97.48      97.45   98.52   98.20   98.71    95.59  93.52   89.58  97.72        98.06  98.94   95.28  96.22
% te_2     99.05  94.47      99.12   99.51   100.00  97.03    98.87  99.34   97.20  98.86        97.24  97.89   95.94  98.04
% te_5     99.81  99.90      99.90   100.00  100.00  100.00   99.44  99.81   98.94  99.90        99.18  99.62   98.11  99.59
% te_10    99.81  100.00     100.00  100.00  100.00  100.00   99.72  99.81   99.61  100.00       99.69  100.00  98.30  99.77
% proj_2   68.38  16.49      25.39   36.91   58.78   24.08    54.18  45.16   36.10  39.20        22.27  31.77   30.41  37.62
% proj_5   96.67  70.81      89.51   92.13   96.61   82.36    95.68  90.33   87.07  93.34        83.04  89.06   86.02  88.66
% proj_10  98.57  92.43      99.31   99.02   99.50   97.52    98.69  97.28   95.95  98.76        95.71  97.41   95.94  97.39
% re       5.67   4.26       4.20    3.43    3.78    3.10     4.91   4.57    6.07   3.94         3.93   3.52    4.24   4.28
% te       0.00   0.01       0.01    0.00    0.00    0.01     0.01   0.00    0.01   0.00         0.01   0.01    0.01   0.01


==> CVPR2023/tbl/quantitative/refine_real275.tex <==

% {\color{red} @yinghan}: TODO: please add the table of catre (real 275) in here. Add the prior and synthetic data mark as well.


\begin{table}[]
\begin{center}

\caption{\textbf{Results of category-level pose on REAL275 using new IoU metric.} Overall best results are in bold and the second
best results are underlined. \emph{Type} lists the type of the input data for
pose estimation. \emph{Syn.} denotes whether synthetic data is used during training. \emph{Prior} denotes whether the method utilizes shape
priors.}
\label{tbl:cat_perform_CATRE}
\vspace{-3mm}
\resizebox{\linewidth}{!}
{%

\begin{tabular}{@{}r|c|c|c|c|cccc@{}}
\toprule

Method      &  Type & Syn. & Prior & $\text{IoU}_{75}$ & $5^\circ 2\text{cm}$ & $5^\circ 5\text{cm}$ & $10^\circ 2\text{cm}$ & $10^\circ 5\text{cm}$ \\
\midrule
\midrule            
NOCS \cite{NOCS_2019_CVPR} & RGB-D & \checkmark & \checkmark & 9.4   & 7.2  & 10.0 & 13.8  & 25.2  \\
CR-Net \cite{CR-Net_2021_IROS} & RGB-D & \checkmark & \checkmark & 33.2  & 27.8 & 34.3 & 47.2  & 60.8  \\
SGPA \cite{SGPA_2021_ICCV} & RGB-D & \checkmark & \checkmark & {37.1}  & {35.9} & 39.6 & {61.3}  & 70.7  \\
Self-DPDN \cite{Self-DPDN_ECCV_2022} & RGB-D & \checkmark & \checkmark & \textbf{42.2}  &\underline{44.3} & \underline{50.9}  &\underline{65.1} & {78.6} \\
SPD  \cite{Tian_ShapePrior_2020_ECCV} & RGB-D & \checkmark & \checkmark  & 27.0  & 19.3 & 21.4 & 43.2  & 54.1  \\
RBP-Pose \cite{RBP-Pose_ECCV_2022} & D & & \checkmark & 24.5 & 38.38 & {48.28} & {63.28} & \underline{79.56}\\
GPV-Pose \cite{GPV-Pose_2022_CVPR} & D & & & 23.1 & 32.7 & {41.8} & 57.2 & {74.9} \\ 
\midrule
\textbf{HS-Pose (Ours)} & D & & & \underline{39.1} & \textbf{46.7} & \textbf{55.4} & \textbf{69.8} & \textbf{82.9}\\ 
% \midrule
% DualPoseNet \cite{DualPoseNet_2021_ICCV} &  \checkmark & RGB-D & \checkmark & \checkmark & 30.8  & 29.3 & 35.9 & 50    & 66.8  \\
% SPD  \cite{liu_2022_catre} &  \checkmark & RGB-D & \checkmark & \checkmark & \underline{43.6}  & \underline{45.8} & {54.4} & \underline{61.4}  & 73.1  \\
% % RBP-Pose \cite{RBP-Pose_ECCV_2022} & \checkmark & D & & \checkmark & 38.6 & 40.4 & \underline{54.8} & 55.8 & {78.1}\\
% GPV-Pose & \checkmark & D & & & 40.7 & 39.9 & 54.3 & 57.3 & \underline{79.1} \\
% \textbf{HS-Pose (Ours)} & \checkmark & D & & & \textbf{47.6} & \textbf{48.4} & \textbf{58.1} & \textbf{67.0} & \textbf{79.5} \\
\bottomrule
\end{tabular}
}

\end{center}
\end{table}

% -------------SelfDPDN no refine ----------------
% [1121_130414 core.catre.engine.catre_custom_evaluator@84]: load gts of nocs_test_real
% 100%|##########| 2754/2754 [00:00<00:00, 29228.60it/s]
% 2754it [00:38, 70.71it/s] 
% [1121_130453 core.catre.engine.catre_custom_evaluator@318]: 
% objects   bottle  bowl    camera  can    laptop  mug     Avg(6)
% IoU25     51.63   99.99   90.74   71.38  85.50   99.64   83.15
% IoU50     49.31   99.99   80.83   71.14  82.86   99.04   80.53
% IoU75     30.23   92.20   19.72   33.71  76.58   0.58    42.17
% re5te2    46.45   87.03   0.21    62.48  60.20   9.65    44.34
% re5te5    49.29   92.77   0.23    64.65  76.89   21.52   50.89
% re10te2   78.95   93.82   6.67    93.88  68.73   48.78   65.14
% re10te5   87.08   100.00  7.41    98.89  93.93   84.18   78.58
% re10te10  99.00   100.00  7.41    98.93  96.06   84.18   80.93
% re5       67.93   92.83   0.24    68.12  77.82   21.52   54.74
% re10      99.00   100.00  7.96    98.93  96.11   84.18   81.03
% te2       79.46   93.82   69.62   94.38  68.80   58.57   77.44
% te5       88.23   100.00  99.66   99.68  95.28   100.00  97.14

% -------------RBP-Pose no refine ----------------
% [1128_102336 core.catre.engine.catre_custom_evaluator@84]: load gts of nocs_test_real
% 100%|##########| 2754/2754 [00:00<00:00, 29683.70it/s]
% 2754it [00:39, 69.96it/s] 
% [1128_102416 core.catre.engine.catre_custom_evaluator@318]: 
% objects   bottle  bowl    camera  can    laptop  mug     Avg(6)
% IoU25     56.39   99.99   90.63   71.41  86.38   99.64   84.07
% IoU50     16.14   99.43   69.08   70.96  85.57   95.38   72.76
% IoU75     0.00    68.13   3.54    11.37  27.37   36.58   24.50
% re5te2    37.94   76.09   1.34    54.38  41.22   19.29   38.38
% re5te5    43.22   81.88   1.59    68.08  75.06   19.84   48.28
% re10te2   76.19   91.86   21.48   79.82  44.32   66.03   63.28
% re10te5   90.98   99.94   26.84   97.70  94.16   67.73   
% re10te10  96.41   99.94   27.05   97.74  97.90   67.73   81.13
% re5       50.40   83.62   1.78    69.76  77.71   19.85   50.52
% re10      98.02   99.94   28.93   98.00  97.90   67.74   81.75
% te2       79.84   91.93   63.02   81.84  44.32   97.02   76.33
% te5       95.01   100.00  97.59   99.88  94.42   100.00  97.82

% ----------- RBP-Pose refined with 2 iters refine ----------------
% [1128_102455 core.catre.engine.catre_custom_evaluator@221]: Eval recalls of results at iter=2...
% 2754it [00:42, 65.31it/s] 
% [1128_102538 core.catre.engine.catre_custom_evaluator@318]: 
% objects   bottle  bowl    camera  can    laptop  mug     Avg(6)
% IoU25     57.66   99.99   90.62   71.46  86.38   99.64   84.29
% IoU50     49.56   99.99   77.83   71.30  85.21   99.04   80.49
% IoU75     3.45    90.23   8.23    30.50  58.13   54.85   40.90
% re5te2    13.80   90.62   1.95    55.54  54.09   21.85   39.64
% re5te5    46.23   95.05   2.00    75.06  81.12   22.17   53.60
% re10te2   30.56   95.42   18.24   77.22  57.64   67.42   57.75
% re10te5   96.05   100.00  20.45   99.65  94.05   69.36   79.93
% re10te10  99.47   100.00  20.59   99.70  94.76   69.36   80.65
% re5       62.56   95.58   2.03    77.25  81.28   22.17   56.81
% re10      99.47   100.00  20.71   99.70  94.89   69.36   80.69
% te2       30.63   95.42   54.32   77.22  58.07   95.97   68.60
% te5       96.41   100.00  97.37   99.96  96.13   100.00  98.31


% ----------- GPV-Pose no refine ----------------
% [1115_113617 core.catre.engine.catre_custom_evaluator@318]: 
% objects   bottle  bowl    camera  can    laptop  mug     Avg(6)
% IoU25     56.73   99.99   90.67   71.46  86.38   99.64   84.15
% IoU50     14.92   99.49   67.29   70.51  84.41   98.75   72.56
% IoU75     0.00    63.68   1.74    15.50  24.18   33.55   23.11
% re5te2    36.56   66.24   0.74    50.76  35.30   6.71    32.72
% re5te5    44.04   73.54   0.97    61.03  63.63   7.44    41.77
% re10te2   72.92   88.35   11.17   82.61  39.90   48.02   57.16
% re10te5   91.16   99.85   14.47   98.01  91.08   54.88   74.91
% re10te10  97.66   99.85   14.68   98.01  95.66   54.88   76.79
% re5       55.17   75.13   1.02    63.36  66.14   7.44    44.71
% re10      98.27   99.85   15.83   98.42  95.75   54.95   77.18
% te2       74.56   88.59   61.32   84.16  40.02   85.49   72.36
% te5       93.77   100.00  95.77   99.80  93.58   100.00  97.15

% ----------- GPV-Pose refined with 2 iters refine ----------------
% [1115_113748 core.catre.engine.catre_custom_evaluator@318]: 
% objects   bottle  bowl    camera  can    laptop  mug     Avg(6)
% IoU25     57.66   99.99   90.70   71.46  86.35   99.64   84.30
% IoU50     50.23   99.99   75.86   71.09  84.67   99.09   80.15
% IoU75     2.78    90.71   5.47    28.66  53.47   63.09   40.70
% re5te2    16.38   89.74   1.46    57.20  53.35   21.33   39.91
% re5te5    49.93   94.23   1.47    76.33  81.96   21.62   54.26
% re10te2   32.16   95.30   11.35   77.49  56.82   70.46   57.26
% re10te5   95.98   100.00  12.67   99.55  93.97   72.24   79.07
% re10te10  99.51   100.00  12.75   99.55  94.53   72.24   79.76
% re5       63.48   95.22   1.48    78.40  82.01   21.62   57.04
% re10      99.51   100.00  12.75   99.55  94.53   72.24   79.76
% te2       32.23   95.30   53.54   77.49  57.18   97.53   68.88
% te5       96.30   100.00  96.97   99.88  96.22   100.00  98.23

% ----------- HS-Pose (ours) no refine ----------------
% [1115_111756 core.catre.engine.catre_custom_evaluator@318]: 
% objects   bottle  bowl    camera  can    laptop  mug    Avg(6)
% IoU25     57.41   99.99   89.83   71.41  86.38   99.64  84.11
% IoU50     50.85   99.99   70.17   71.14  84.63   98.26  79.17
% IoU75     24.11   87.03   10.65   33.88  59.97   18.91  39.09
% re5te2    43.12   92.09   2.28    69.39  49.23   23.77  46.65
% re5te5    53.31   95.58   3.10    75.82  79.51   24.96  55.38
% re10te2   80.19   96.45   28.25   91.18  52.39   70.42  69.82
% re10te5   95.62   100.00  35.71   99.68  93.97   72.58  82.93
% re10te10  98.99   100.00  35.79   99.68  96.74   72.58  83.96
% re5       66.86   95.58   3.11    77.93  80.75   24.96  58.20
% re10      99.19   100.00  35.79   99.68  96.82   72.59  84.01
% te2       81.21   96.45   60.90   91.18  52.39   96.38  79.75
% te5       96.80   100.00  98.09   99.80  94.52   99.89  98.18

% ----------- HS-Pose (ours) refined with 2 iters ----------------
% [1115_111835 core.catre.engine.catre_custom_evaluator@221]: Eval recalls of results at iter=2...
% 2754it [00:38, 71.29it/s] 
% [1115_111914 core.catre.engine.catre_custom_evaluator@318]: 
% objects   bottle  bowl    camera  can    laptop  mug     Avg(6)
% IoU25     56.62   99.99   89.73   71.46  86.08   99.64   83.92
% IoU50     50.39   99.99   73.12   71.22  83.09   98.56   79.40
% IoU75     21.78   91.39   7.12    35.24  66.45   63.84   47.63
% re5te2    52.24   91.30   1.35    71.55  53.00   21.22   48.44
% re5te5    62.77   96.74   1.35    83.77  81.78   21.96   58.06
% re10te2   81.43   94.45   13.05   84.58  56.89   71.55   66.99
% re10te5   95.16   100.00  14.31   99.57  93.90   74.25   79.53
% re10te10  99.83   100.00  14.40   99.66  95.08   74.25   80.54
% re5       77.50   96.77   1.36    85.18  81.94   21.96   60.78
% re10      99.83   100.00  14.40   99.66  95.08   74.29   80.55
% te2       81.43   94.45   53.87   84.58  57.17   97.00   78.08
% te5       95.28   100.00  97.03   99.80  95.90   100.00  98.00

% 57.41   99.99   89.83   71.41  86.38   99.64  84.11
% 50.85   99.99   70.17   71.14  84.63   98.26  79.17
% 24.11   87.03   10.65   33.88  59.97   18.91  39.09
% 43.12   92.09   2.28    69.39  49.23   23.77  46.65
% 53.31   95.58   3.10    75.82  79.51   24.96  55.38
% 80.19   96.45   28.25   91.18  52.39   70.42  69.82
% 95.62   100.00  35.71   99.68  93.97   72.58  82.93
% 98.99   100.00  35.79   99.68  96.74   72.58  83.96
% 66.86   95.58   3.11    77.93  80.75   24.96  58.20
% 99.19   100.00  35.79   99.68  96.82   72.59  84.01
% 81.21   96.45   60.90   91.18  52.39   96.38  79.75
% 96.80   100.00  98.09   99.80  94.52   99.89  98.18

==> CVPR2023/tbl/quantitative/results_real275_table_IOUfixed.tex <==

\begin{table*}[ht]
\begin{center}

\caption{\textbf{Per-category results of our method on REAL275 dataset.} }
% \label{tbl:cat_perform}
\vspace{-3mm}
\resizebox{0.8\linewidth}{!}
{%

\begin{tabular}{@{}c|ccc|ccccc|cc|ccc@{}}
\toprule

category & $\text{IoU}_{25}$ & $\text{IoU}_{50}$ & $\text{IoU}_{75}$ & $5^\circ 2\text{cm}$ & $5^\circ 5\text{cm}$ & $10^\circ 2\text{cm}$ & $10^\circ 5\text{cm}$ & $10^\circ 10\text{cm}$ & $5^\circ $   & $10^\circ $   & $2$cm   & $5$cm    & $10$cm   \\ 
\midrule
\midrule            
bottle   & 57.7  & 57.7  & 54.8  & 43.0 & 53.1 & 80.0  & 95.4  & 98.5   & 66.9 & 99.2  & 81.0 & 96.5  & 99.5  \\
bowl     & 100.0 & 100.0 & 100.0 & 92.1 & 95.6 & 96.5  & 100.0 & 100.0  & 95.6 & 100.0 & 96.5 & 100.0 & 100.0 \\
camera   & 90.9  & 82.3  & 65.2  & 2.3  & 3.1  & 28.3  & 35.7  & 35.8   & 3.1  & 35.8  & 60.9 & 98.1  & 100.0 \\
can      & 71.4  & 71.4  & 70.5  & 68.6 & 75.0 & 90.0  & 98.5  & 98.5   & 77.8 & 99.7  & 90.0 & 98.6  & 98.8  \\
laptop   & 86.1  & 84.9  & 67.1  & 49.3 & 79.5 & 52.4  & 94.0  & 96.8   & 80.8 & 96.9  & 52.4 & 94.6  & 99.5  \\
mug      & 99.2  & 96.4  & 90.8 & 23.8 & 25.0 & 64.6  & 72.6  & 72.6   & 25.0 & 72.6  & 88.5 & 100.0 & 100.0 \\ \midrule
average  & 84.2  & 82.1  & 74.7  & 46.5 & 55.2 & 68.6  & 82.7  & 83.7   & 58.2 & 84.0  & 78.2 & 98.0  & 99.6  \\ \bottomrule
\end{tabular}
}
\end{center}
\end{table*}

==> CVPR2023/tex/gcn3d.tex <==
\section{Background: 3D Graph Convolution}\label{sec:3dgc}
Since the proposed method is strongly related to 3D graph convolution (3D-GC), we briefly review its implementation here.
%
3D graph convolution (3D-GC), as proposed in \cite{3dgcn_lin_CVPR_2020}, is a neural network structure designed to extract local geometric features from unordered point cloud data. Since distinguishing deterministic geometric features is usually needed to recover an object's pose from various shapes, 3D-GC has recently gained popularity in the category-level object pose estimation domain \cite{FSNET_2021_CVPR, GPV-Pose_2022_CVPR, SSP-Pose_IROS_22, SAR-Net_Lin_2022_CVPR, RBP-Pose_ECCV_2022}. 

The input to 3D-GC is the point cloud and the features associated with the points $\{(\point_n\in\realR^3, \feature_n \in \realR^{D_\text{in}})\}_{n=1}^N$. The output of 3D-GC is the point cloud with their extracted features $\{(\point_n\in\realR^3,\feature_n \in \realR^{D_\text{out}})\}_{n=1}^N$, possibly with a different feature dimension.

The core unit of 3D-GC is a deformable kernel that generalizes the convolution kernel used in 2D image processing to deal with unstructured point cloud data. In particular, a 3D-GC kernel $K^S$ is defined as:
\begin{equation}
    K^S = \{(\kernelPoint_C, \weight_C), (\kernelPoint_1, \weight_1), \dots, (\kernelPoint_S, \weight_S)\},
\end{equation}
where $S$ is the total number of support vectors, $\kernelPoint_C=[0, 0, 0]^T$ is the central kernel point, $\{\kernelPoint_s\in \realR^3\}_{s=1}^N$ are the support kernel vectors and ${\weight}$ is the weight associated with each kernel vector. The 3D-GC kernel performs a convolution on the receptive field $R^M(\point_i)$, which is the point along with its neighbors and their associated features $\feature$:
\begin{equation}
    \label{eq:receptive_field}
    R^M(\point_i) = \{(\point_i, \feature_i), (\point_m, \feature_m) | \point_m \in \neighbor^M(\point_i)\}.
\end{equation}
Here $\neighbor^M(\point_i)$ is the set of the $M$ nearest neighbor points of $\point_i$. In particular, in \cite{3dgcn_lin_CVPR_2020} the receptive field with point distance metric (RF-P) is used for finding which of the nearest neighbors is within the point distance metric:
\begin{equation}
  \distance_p(\point_i, \point_j) = \norm{\point_i - \point_j}.
\end{equation}

% In particular, $\neighbor^M(\point_i)$ is defined as a set of points that satisfies:
% \begin{align*}
%     &\neighbor^M(\point_i) \subseteq \pointCloud,
%     |\neighbor^M(\point_i)| = M \text{ and } \\
%     &\text{for all } \point_n \in \pointCloud \setminus \neighbor^M(\point_i), \text{ we have} \\
%     &\distance(\point_i, \point_n) \geq \max_{\point_m \in \neighbor^M(\point_i)} \distance(\point_i, \point_m)  
% \end{align*}
% where $|\cdot|$ measures the cardinal number of a set, and $\distance(\cdot, \cdot)$ is a valid distance metric. 

% %It should be noticed that the number of support kernel points $S$ and the number of neighbors in the receptive field $M$ could be different, and both of them are hyperparameters that can be tuned.

The convolution between the receptive field $R^M(\point_i)$ and the 3D-GC kernel $K^S$ is defined as:
\begin{equation}
    \convolution(R^M(\point_i), K^S) = \feature_i^T\weight_C + 
    \sum_{s=1}^{S} \max_{\point_m \in \neighbor^M(\point_i)} \similarity(\point_m, \kernelPoint_s),
    \label{eq:gc}
\end{equation}
% \begin{equation}
% \begin{aligned}
%     \convolution(R^M(\point_i), K^S) = &\feature_i^T\weight_C \\ &+ 
%     \sum_{s=1}^{S} \max_{\point_m \in \neighbor^M(\point_i)} \similarity(\point_m, \kernelPoint_s)
%     \label{eq:gc}
% \end{aligned}
% \end{equation}
where $\similarity(\point_m, \kernelPoint_s)$ measures the similarity between the neighbor point $\point_m$ and the kernel support vector $\kernelPoint_s$:
\begin{equation}
    \similarity(\point_m, \kernelPoint_s) =
    \feature_m^T\weight_s \frac{(\point_m - \point_i)^T\kernelPoint_s}{\norm{\point_m - \point_i}\norm{\kernelPoint_s}}
    \label{eq:sim}.
\end{equation}
% For the first layer of graph convolution where the points the do not have corresponding features, $\feature_n$ and the $\weight$ for kernel are set to $1$.

It should be noted that 3D-GC has a size and translation invariance due to the normalization in Eq.~\ref{eq:sim}. A brief inner structure of the 3D-GC layer is shown in Fig.~\ref{fig:gcn3d}. For more details, the readers can refer to the original work \cite{3dgcn_lin_CVPR_2020}. 
\input{CVPR2023/fig/3dgcn_structure/item.tex}
% With the 3D-GC kernel and receptive field, the 3D-GC Convolution layer and 3D Graph max pooling can be constructed to form the 3D-GC network (3D-GCN) \cite{3dgcn_lin_CVPR_2020}, which has shown superior local geometric perception and brought impressive performance improvement in category-level object pose estimation tasks \cite{FSNET_2021_CVPR, GPV-Pose_2022_CVPR, RBP-Pose_ECCV_2022}. However, 
% It should be noticed that the scale and translation invariance of 3D-GC conflicts with category-level pose estimation tasks, which are required to estimate the object's translation and size. Also, looking only at the local regions makes 3D-GC unable to perceive the global geometric structural relationships and, consequently, is sensitive to noise as well as showing a limited ability to handle complex shapes. In this work, we will show how simple modifications of the 3D-GC net can significantly improve the three problems mentioned above.



==> supbib.tex <==
@String(PAMI = {IEEE Trans. Pattern Anal. Mach. Intell.})
@String(IJCV = {Int. J. Comput. Vis.})
@String(CVPR= {IEEE Conf. Comput. Vis. Pattern Recog.})
@String(ICCV= {Int. Conf. Comput. Vis.})
@String(ECCV= {Eur. Conf. Comput. Vis.})
@String(NIPS= {Adv. Neural Inform. Process. Syst.})
@String(ICPR = {Int. Conf. Pattern Recog.})
@String(BMVC= {Brit. Mach. Vis. Conf.})
@String(TOG= {ACM Trans. Graph.})
@String(TIP  = {IEEE Trans. Image Process.})
@String(TVCG  = {IEEE Trans. Vis. Comput. Graph.})
@String(TMM  = {IEEE Trans. Multimedia})
@String(ACMMM= {ACM Int. Conf. Multimedia})
@String(ICME = {Int. Conf. Multimedia and Expo})
@String(ICASSP=	{ICASSP})
@String(ICIP = {IEEE Int. Conf. Image Process.})
@String(ACCV  = {ACCV})
@String(ICLR = {Int. Conf. Learn. Represent.})
@String(IJCAI = {IJCAI})
@String(PR   = {Pattern Recognition})
@String(AAAI = {AAAI})
@String(CVPRW= {IEEE Conf. Comput. Vis. Pattern Recog. Worksh.})
@String(CSVT = {IEEE Trans. Circuit Syst. Video Technol.})

@String(SPL	= {IEEE Sign. Process. Letters})
@String(VR   = {Vis. Res.})
@String(JOV	 = {J. Vis.})
@String(TVC  = {The Vis. Comput.})
@String(JCST  = {J. Comput. Sci. Tech.})
@String(CGF  = {Comput. Graph. Forum})
@String(CVM = {Computational Visual Media})


@String(PAMI  = {IEEE TPAMI})
@String(IJCV  = {IJCV})
@String(CVPR  = {CVPR})
@String(ICCV  = {ICCV})
@String(ECCV  = {ECCV})
@String(NIPS  = {NeurIPS})
@String(ICPR  = {ICPR})
@String(BMVC  =	{BMVC})
@String(TOG   = {ACM TOG})
@String(TIP   = {IEEE TIP})
@String(TVCG  = {IEEE TVCG})
@String(TCSVT = {IEEE TCSVT})
@String(TMM   =	{IEEE TMM})
@String(ACMMM = {ACM MM})
@String(ICME  =	{ICME})
@String(ICASSP=	{ICASSP})
@String(ICIP  = {ICIP})
@String(ACCV  = {ACCV})
@String(ICLR  = {ICLR})
@String(IJCAI = {IJCAI})
@String(PR = {PR})
@String(AAAI = {AAAI})
@String(CVPRW= {CVPRW})
@String(CSVT = {IEEE TCSVT})



@misc{Authors14,
 author = {FirstName LastName},
 title = {The frobnicatable foo filter},
 note = {Face and Gesture submission ID 324. Supplied as supplemental material {\tt fg324.pdf}},
 year = 2014
}

@misc{Authors14b,
 author = {FirstName LastName},
 title = {Frobnication tutorial},
 note = {Supplied as supplemental material {\tt tr.pdf}},
 year = 2014
}

@article{Alpher02,
author = {FirstName Alpher},
title = {Frobnication},
journal = PAMI,
volume = 12,
number = 1,
pages = {234--778},
year = 2002
}

@article{Alpher03,
author = {FirstName Alpher and  FirstName Fotheringham-Smythe},
title = {Frobnication revisited},
journal = {Journal of Foo},
volume = 13,
number = 1,
pages = {234--778},
year = 2003
}

@article{Alpher04,
author = {FirstName Alpher and FirstName Fotheringham-Smythe and FirstName Gamow},
title = {Can a machine frobnicate?},
journal = {Journal of Foo},
volume = 14,
number = 1,
pages = {234--778},
year = 2004
}

@inproceedings{Alpher05,
author = {FirstName Alpher and FirstName Gamow},
title = {Can a computer frobnicate?},
booktitle = CVPR,
pages = {234--778},
year = 2005
}

@InProceedings{NOCS_2019_CVPR,
author = {Wang, He and Sridhar, Srinath and Huang, Jingwei and Valentin, Julien and Song, Shuran and Guibas, Leonidas J.},
title = {Normalized Object Coordinate Space for Category-Level 6D Object Pose and Size Estimation},
booktitle = {The IEEE Conference on Computer Vision and Pattern Recognition (CVPR)},
month = {June},
year = {2019}
}

@inproceeding{OPT2017,
    author    = {Wu, Po-Chen and Lee, Yueh-Ying and Tseng, Hung-Yu and Ho, Hsuan-I and Yang, Ming-Hsuan and Chien, Shao-Yi}, 
    title     = {A Benchmark Dataset for 6DoF Object Pose Tracking}, 
    booktitle = {IEEE International Symposium on Mixed and Augmented Reality (ISMAR Adjunct)},
    year      = {2017}
}

@inproceedings{YCB_M_2020,
author = {Grenzdörffer, Till and Günther, Martin and Hertzberg, Joachim},
year = {2020},
month = {May},
pages = {},
title = {{YCB-M: A Multi-Camera RGB-D Dataset for Object Recognition and 6DoF Pose Estimation}},
booktitle= {International Conference on Robotics and Automation (ICRA)}
}

@inproceedings{6D_Rotation_2019_CVPR,
author = {Zhou, Yi and Barnes, Connelly and Lu, Jingwan and Yang, Jimei and Li, Hao},
year = {2019},
month = {06},
pages = {5738-5746},
title = {{On the Continuity of Rotation Representations in Neural Networks}},
doi = {10.1109/CVPR.2019.00589},
booktitle = {IEEE Conference on Computer Vision and Pattern Recognition (CVPR)}
}

@article{AAE_perspective,
author = {Sundermeyer, Martin and Marton, Zoltan and Durner, Maximilian and Triebel, Rudolph},
year = {2019},
month = {10},
pages = {},
title = {{Augmented Autoencoders: Implicit 3D Orientation Learning for 6D Object Detection}},
volume = {128},
journal = {International Journal of Computer Vision (IJCV)},
doi = {10.1007/s11263-019-01243-8}
}

@inproceedings{CosyPose_ECCV_2020,
author = {Labbé, Yann and Carpentier, Justin and Aubry, Mathieu and Sivic, Josef},
year = {2020},
month = {August},
pages = {},
title = {{CosyPose: Consistent multi-view multi-object 6D pose estimation}},
booktitle={Proceedings of the European Conference on Computer Vision (ECCV)},
}

@unknown{category_level_2,
author = {Sahin, Caner and Kim, Tae-Kyun},
year = {2018},
month = {08},
pages = {},
title = {Category-level 6D Object Pose Recovery in Depth Images}
}

@article{Review_Object_Pose_Recovery,
title = "A review on object pose recovery: From 3D bounding box detectors to full 6D pose estimators",
journal = "Image and Vision Computing",
pages = "103898",
year = "2020",
issn = "0262-8856",
doi = "https://doi.org/10.1016/j.imavis.2020.103898",
url = "http://www.sciencedirect.com/science/article/pii/S0262885620300305",
author = "Caner Sahin and Guillermo Garcia-Hernando and Juil Sock and Tae-Kyun Kim",
}

@inproceedings{BOP,
author = {Hodan, Tomas and Michel, Frank and Brachmann, Eric and Kehl, Wadim and Buch, Anders and Kraft, Dirk and Drost, Bertram and Vidal, Joel and Ihrke, Stephan and Zabulis, Xenophon and Sahin, Caner and Manhardt, Fabian and Tombari, Federico and Kim, Tae-Kyun and Matas, Jiří and Rother, Carsten},
year = {2018},
pages = {19-35},
title = {{BOP: Benchmark for 6D Object Pose Estimation: 15th European Conference, Munich, Germany, September 8-14, Proceedings, Part X}},
isbn = {978-3-030-01248-9},
doi = {10.1007/978-3-030-01249-6_2}
}

@InProceedings{Refinement_CNN_Krull_2015_ICCV,
author = {Krull, Alexander and Brachmann, Eric and Michel, Frank and Ying Yang, Michael and Gumhold, Stefan and Rother, Carsten},
title = {Learning Analysis-by-Synthesis for 6D Pose Estimation in RGB-D Images},
booktitle = {The IEEE International Conference on Computer Vision (ICCV)},
month = {December},
year = {2015}
}

@inproceedings{OneShot_2d3d_2022_CVPR,
  title={OnePose: One-Shot Object Pose Estimation without CAD Models},
  author={Sun, Jiaming and Wang, Zihao and Zhang, Siyu and He, Xingyi and Zhao, Hongcheng and Zhang, Guofeng and Zhou, Xiaowei},
  booktitle={Proceedings of the IEEE/CVF Conference on Computer Vision and Pattern Recognition},
  pages={6825--6834},
  year={2022}
}

@inproceedings{Uni6d_2022_CVPR,
  title={Uni6D: A Unified CNN Framework without Projection Breakdown for 6D Pose Estimation},
  author={Jiang, Xiaoke and Li, Donghai and Chen, Hao and Zheng, Ye and Zhao, Rui and Wu, Liwei},
  booktitle={Proceedings of the IEEE/CVF Conference on Computer Vision and Pattern Recognition},
  pages={11174--11184},
  year={2022}
}

@InProceedings{Synthetic_Real_Data_Papon_2015_ICCV,
author = {Papon, Jeremie and Schoeler, Markus},
title = {Semantic Pose Using Deep Networks Trained on Synthetic RGB-D},
booktitle = {The IEEE International Conference on Computer Vision (ICCV)},
month = {December},
year = {2015}
}

@article{T_Less_hodan_2017_WACV,
  title={{T-LESS}: An {RGB-D} Dataset for {6D} Pose Estimation of Texture-less Objects},
  author={Hoda{\v{n}}, Tom{\'a}{\v{s}} and Haluza, Pavel and Obdr{\v{z}}{\'a}lek, {\v{S}}t{\v{e}}p{\'a}n and Matas, Ji{\v{r}}{\'\i} and Lourakis, Manolis and Zabulis, Xenophon},
  journal={IEEE Winter Conference on Applications of Computer Vision (WACV)},
  year={2017}
}

@InProceedings{OCC_LINEMOD_2014_ECCV,
author="Brachmann, Eric
and Krull, Alexander
and Michel, Frank
and Gumhold, Stefan
and Shotton, Jamie
and Rother, Carsten",
editor="Fleet, David
and Pajdla, Tomas
and Schiele, Bernt
and Tuytelaars, Tinne",
title="Learning 6D Object Pose Estimation Using 3D Object Coordinates",
booktitle="Computer Vision -- ECCV 2014",
year="2014",
publisher="Springer International Publishing",
address="Cham",
pages="536--551",
isbn="978-3-319-10605-2"
}

@InProceedings{VSD_Hoda_2016,
author="Hoda{\v{n}}, Tom{\'a}{\v{s}}
and Matas, Ji{\v{r}}{\'i}
and Obdr{\v{z}}{\'a}lek, {\v{S}}t{\v{e}}p{\'a}n",
title={{On Evaluation of 6D Object Pose Estimation}},
booktitle="ECCV 2016 Workshops",
year="2016",
pages="606--619",
isbn="978-3-319-49409-8"
}

@inproceedings{Hodan_textureless_2015_IROS,
author = {Hodan, Tomas and Zabulis, Xenophon and Lourakis, Manolis and Obdrzalek, Stepan and Matas, Jiri},
year = {2015},
month = {09},
pages = {4421-4428},
title = {Detection and fine 3D pose estimation of texture-less objects in RGB-D images},
doi = {10.1109/IROS.2015.7354005}
}

@inproceedings{HopeNet_2020_CVPR, 
    title = {{HOPE-Net: A Graph-based Model for Hand-Object Pose Estimation}},
    author = {Bardia Doosti and Shujon Naha and Majid Mirbagheri and David Crandall},
    year = {2020},
    booktitle = {IEEE Conference on Computer Vision and Pattern Recognition (CVPR)}
}

@inproceedings{HO_2019_CVPR,
    author = {Tekin, Bugra and Bogo, Federica and Pollefeys, Marc},
    year = {2019},
    month = {06},
    pages = {4506-4515},
    title = {{H+O: Unified Egocentric Recognition of 3D Hand-Object Poses and Interactions}},
    doi = {10.1109/CVPR.2019.00464},
    booktitle = {IEEE Conference on Computer Vision and Pattern Recognition (CVPR)}
}

@INPROCEEDINGS{HO3D,
    title={{HOnnotate: A method for 3D Annotation of Hand and Object Poses}},
    author={Shreyas Hampali and Mahdi Rad and Markus Oberweger and Vincent Lepetit},
    booktitle = {IEEE Conference on Computer Vision and Pattern Recognition (CVPR)},
    year = {2020}
}

@misc{sahin2018categorylevel,
      title={Category-level 6D Object Pose Recovery in Depth Images}, 
      author={Caner Sahin and Tae-Kyun Kim},
      year={2018},
      eprint={1808.00255},
      archivePrefix={arXiv},
      primaryClass={cs.CV}
}

@inproceedings{Frank2015KinematciChain,
author = {Michel, Frank and Krull, Alexander and Brachmann, Eric and Yang, Michael Ying and Gumhold, Stefan and Rother, Carsten},
year = {2015},
month = {09},
pages = {},
title = {Pose Estimation of Kinematic Chain Instances via Object Coordinate Regression},
doi = {10.5244/C.29.181}
}
@article{In_Hand_Pose_2016_RAL,
author = {Bimbo, Joao and Luo, Shan and Althoefer, Kaspar and Liu, Hongbin},
year = {2016},
month = {01},
pages = {1-1},
title = {In-Hand Object Pose Estimation Using Covariance-Based Tactile To Geometry Matching},
volume = {1},
journal = {IEEE Robotics and Automation Letters},
doi = {10.1109/LRA.2016.2517244}
}

@InProceedings{EPOS_2020_CVPR,
author = {Hodan, Tomas and Barath, Daniel and Matas, Jiri},
title = {EPOS: Estimating 6D Pose of Objects With Symmetries},
booktitle = {Proceedings of the IEEE/CVF Conference on Computer Vision and Pattern Recognition (CVPR)},
month = {June},
year = {2020}
}

@article{RANSAC,
  added-at = {2013-12-10T15:04:12.000+0100},
  author = {Fischler, M. and Bolles, R.},
  biburl = {https://www.bibsonomy.org/bibtex/2cf7f4278e6687a425dbe2374f5b84d07/anas.razeq},
  interhash = {8a99a961293d8dfe59a1f0838d77a24a},
  intrahash = {cf7f4278e6687a425dbe2374f5b84d07},
  journal = { Communications of the ACM},
  keywords = {RANSAC},
  number = { 6},
  pages = { 381-395},
  timestamp = {2013-12-10T15:04:12.000+0100},
  title = {{Random Sample Consensus: A Paradigm for Model Fitting with Applications to Image Analysis and Automated Cartography}},
  url = {/brokenurl# http://publication.wilsonwong.me/load.php?id=233282275},
  volume = { 24},
  year = { 1981}
}

@InProceedings{ADD_Hinterstoisser_2012_ACCV,
author="Hinterstoisser, Stefan
and Lepetit, Vincent
and Ilic, Slobodan
and Holzer, Stefan
and Bradski, Gary
and Konolige, Kurt
and Navab, Nassir",
title={{Model Based Training, Detection and Pose Estimation of Texture-Less 3D Objects in Heavily Cluttered Scenes}},
booktitle="Asian Conference on Computer Vision (ACCV)",
year="2013",
pages="548--562",
isbn="978-3-642-37331-2"
}

@InProceedings{Densefusion_Wang_2019_CVPR,
author = {Wang, Chen and Xu, Danfei and Zhu, Yuke and Martin-Martin, Roberto and Lu, Cewu and Fei-Fei, Li and Savarese, Silvio},
title = {{DenseFusion: 6D Object Pose Estimation by Iterative Dense Fusion}},
booktitle = {The IEEE Conference on Computer Vision and Pattern Recognition (CVPR)},
month = {June},
year = {2019}
}

@article{Applications_robotic_manipulation_1,
author = {Collet, Alvaro and Martinez, Manuel and Srinivasa, Siddhartha},
year = {2011},
month = {09},
pages = {1284-1306},
title = {{The MOPED framework: Object recognition and pose estimation for manipulation}},
volume = {30},
journal = {International Journal of Robotics Research (IJRR)},
doi = {10.1177/0278364911401765}
}
@unknown{Applications_robotic_manipulation_2,
author = {Tremblay, Jonathan and To, Thang and Sundaralingam, Balakumar and Xiang, Yu and Fox, Dieter and Birchfield, Stan},
year = {2018},
month = {09},
pages = {},
title = {Deep Object Pose Estimation for Semantic Robotic Grasping of Household Objects}
}

@inproceedings{Applications_robotic_manipulation_3,
author = {Zhu, Menglong and Derpanis, Konstantinos and Yang, Yinfei and Brahmbhatt, Samarth and Zhang, Mabel and Phillips, Cody and Lecce, Matthieu and Daniilidis, Kostas},
year = {2014},
month = {05},
pages = {3936-3943},
title = {Single image 3D object detection and pose estimation for grasping},
journal = {Proceedings - IEEE International Conference on Robotics and Automation},
doi = {10.1109/ICRA.2014.6907430}
}

@InProceedings{Application_navigation_1,
author = {Xu, Danfei and Anguelov, Dragomir and Jain, Ashesh},
title = {PointFusion: Deep Sensor Fusion for 3D Bounding Box Estimation},
booktitle = {The IEEE Conference on Computer Vision and Pattern Recognition (CVPR)},
month = {June},
year = {2018}
}

@inproceedings{Application_navigation_2,
author = {Geiger, Andreas},
year = {2012},
month = {06},
pages = {3354-3361},
title = {Are we ready for autonomous driving? The KITTI vision benchmark suite}
}

@inproceedings{Application_navigation_3,
author = {Chen, Xiaozhi and Ma, Huimin and Wan, Ji and Li, Bo and Xia, Tian},
year = {2017},
month = {07},
pages = {6526-6534},
title = {Multi-view 3D Object Detection Network for Autonomous Driving},
doi = {10.1109/CVPR.2017.691}
}

@article{Application_Augmented_Reality_1,
author = {Marchand, Eric and Uchiyama, Hideaki and Spindler, Fabien},
year = {2016},
month = {01},
pages = {},
title = {{Pose Estimation for Augmented Reality: A Hands-On Survey}},
volume = {22},
journal = {IEEE Transactions on Visualization and Computer Graphics},
doi = {10.1109/TVCG.2015.2513408}
}
@inproceedings{Application_Augmented_Reality_2,
author = {Marder-Eppstein, Eitan},
year = {2016},
month = {07},
pages = {25-25},
title = {Project Tango},
doi = {10.1145/2933540.2933550}
}

@article{AR_application_medical_training,
author = {Barsom, E. and Graafland, Maurits and Schijven, Marlies},
year = {2016},
month = {10},
pages = {},
title = {Systematic review on the effectiveness of augmented reality applications in medical training},
volume = {30},
journal = {Surgical Endoscopy},
doi = {10.1007/s00464-016-4800-6}
}

@article{AR_application_manufacturing,
author = {Nee, Andrew and Ong, S K and Chryssolouris, George and Mourtzis, Dimitris},
year = {2012},
month = {12},
pages = {657–679},
title = {{Augmented reality applications in design and manufacturing}},
volume = {61},
journal = {CIRP Annals - Manufacturing Technology},
doi = {10.1016/j.cirp.2012.05.010}
}

@article{AR_application_tourism,
author = {Ozkul, Emrah and Kumlu, Sarp},
year = {2019},
month = {12},
pages = {107-122},
title = {{Augmented Reality Applications in Tourism}},
journal = {International Journal of Contemporary Tourism Research},
doi = {10.30625/ijctr.625192}
}
@article{Posecnn_YCB_Video_Dataset,
author = {Xiang, Yu and Schmidt, Tanner and Narayanan, Venkatraman and Fox, Dieter},
year = {2018},
month = {06},
pages = {},
title = {{PoseCNN: A Convolutional Neural Network for 6D Object Pose Estimation in Cluttered Scenes}},
journal   = {Robotics: Science and Systems (RSS)},
doi = {10.15607/RSS.2018.XIV.019}
}

@INPROCEEDINGS{LineMod, 
author={S. {Hinterstoisser} and S. {Holzer} and C. {Cagniart} and S. {Ilic} and K. {Konolige} and N. {Navab} and V. {Lepetit}}, 
booktitle={International Conference on Computer Vision (ICCV)}, 
title={{Multimodal templates for real-time detection of texture-less objects in heavily cluttered scenes}}, 
year={2011}, 
volume={}, 
number={}, 
pages={858-865}, 
doi={10.1109/ICCV.2011.6126326}, 
ISSN={1550-5499}, 
month={Nov},}


@InProceedings{G2L_Net,
author = {Chen, Wei and Jia, Xi and Chang, Hyung Jin and Duan, Jinming and Leonardis, Ales},
title = {{G2L-Net: Global to Local Network for Real-Time 6D Pose Estimation With Embedding Vector Features}},
booktitle = {IEEE/CVF Conference on Computer Vision and Pattern Recognition (CVPR)},
month = {June},
year = {2020}
}
@inproceedings{SSS_6D_2018_CVPR,
author = {Tekin, Bugra and Sinha, Sudipta and Fua, Pascal},
year = {2018},
month = {06},
pages = {292-301},
title = {Real-Time Seamless Single Shot 6D Object Pose Prediction},
doi = {10.1109/CVPR.2018.00038}
}

@incollection{Latent_3D_Keypoints_NIPS_2018,
title = {Discovery of Latent 3D Keypoints via End-to-end Geometric Reasoning},
author = {Suwajanakorn, Supasorn and Snavely, Noah and Tompson, Jonathan J and Norouzi, Mohammad},
booktitle = {Advances in Neural Information Processing Systems 31},
editor = {S. Bengio and H. Wallach and H. Larochelle and K. Grauman and N. Cesa-Bianchi and R. Garnett},
pages = {2059--2070},
year = {2018},
publisher = {Curran Associates, Inc.},
url = {http://papers.nips.cc/paper/7476-discovery-of-latent-3d-keypoints-via-end-to-end-geometric-reasoning.pdf}
}

@InProceedings{Viewpoints_And_Keypoints_2015_CVPR,
author = {Tulsiani, Shubham and Malik, Jitendra},
title = {Viewpoints and Keypoints},
booktitle = {The IEEE Conference on Computer Vision and Pattern Recognition (CVPR)},
month = {June},
year = {2015}
}

@InProceedings{Implicit_3D_Orientation_2018_ECCV,
author = {Sundermeyer, Martin and Marton, Zoltan-Csaba and Durner, Maximilian and Brucker, Manuel and Triebel, Rudolph},
title = {{Implicit 3D Orientation Learning for 6D Object Detection from RGB Images}},
booktitle = {The European Conference on Computer Vision (ECCV)},
month = {September},
year = {2018}
}

@Article{LSTM_1997,
  author      = {Sepp Hochreiter and Jürgen Schmidhuber},
  journal     = {Neural Computation},
  title       = {{Long Short-Term Memory}},
  year        = {1997},
  number      = {8},
  pages       = {1735--1780},
  volume      = {9},
  optdoi      = {10.1162/neco.1997.9.8.1735},
  opteprint   = {http://dx.doi.org/10.1162/neco.1997.9.8.1735},
  opturl      = {http://dx.doi.org/10.1162/neco.1997.9.8.1735},
}

@inproceedings{GRU_2014,
    title = {{Learning Phrase Representations using {RNN} Encoder{--}Decoder for Statistical Machine Translation}},
    author = {Cho, Kyunghyun  and
      van Merri{\"e}nboer, Bart  and
      Gulcehre, Caglar  and
      Bahdanau, Dzmitry  and
      Bougares, Fethi  and
      Schwenk, Holger  and
      Bengio, Yoshua},
    booktitle = "Proceedings of the 2014 Conference on Empirical Methods in Natural Language Processing ({EMNLP})",
    month = oct,
    year = "2014",
    address = "Doha, Qatar",
    publisher = "Association for Computational Linguistics",
    url = "https://www.aclweb.org/anthology/D14-1179",
    doi = "10.3115/v1/D14-1179",
    pages = "1724--1734",
}

@InProceedings{MCN_2018,
author="Li, Chi
and Bai, Jin
and Hager, Gregory D.",
editor="Ferrari, Vittorio
and Hebert, Martial
and Sminchisescu, Cristian
and Weiss, Yair",
title="A Unified Framework for Multi-view Multi-class Object Pose Estimation",
booktitle="Computer Vision -- ECCV 2018",
year="2018",
publisher="Springer International Publishing",
address="Cham",
pages="263--281",
}

@InProceedings{PoseRBPF, 
    AUTHOR    = {Xinke Deng AND Arsalan Mousavian AND Yu Xiang AND Fei Xia AND Timothy Bretl AND Dieter Fox}, 
    TITLE     = {{PoseRBPF: A Rao-Blackwellized Particle Filter for6D Object Pose Estimation}}, 
    BOOKTITLE = {Proceedings of Robotics: Science and Systems}, 
    YEAR      = {2019}, 
    ADDRESS   = {FreiburgimBreisgau, Germany}, 
    MONTH     = {June}, 
    DOI       = {10.15607/RSS.2019.XV.049} 
}

@inbook{Rao_Blackwellised_Particle_Filter_2001,
	Address = {New York, NY},
	Author = {Murphy, Kevin and Russell, Stuart},
	Booktitle = {Sequential Monte Carlo Methods in Practice},
	Doi = {10.1007/978-1-4757-3437-9_24},
	Isbn = {978-1-4757-3437-9},
	Pages = {499--515},
	Publisher = {Springer New York},
	Title = {Rao-Blackwellised Particle Filtering for Dynamic Bayesian Networks},
	Url = {https://doi.org/10.1007/978-1-4757-3437-9_24},
	Year = {2001},
	Bdsk-Url-1 = {https://doi.org/10.1007/978-1-4757-3437-9_24},
	Bdsk-Url-2 = {http://dx.doi.org/10.1007/978-1-4757-3437-9_24}}

@inproceedings{SE3_TrackNet_2020_IROS,
author = {Wen, Bowen and Mitash, Chaitanya and Ren, Baozhang and Bekris, Kostas},
year = {2020},
month = {07},
pages = {},
title = {{se(3)-TrackNet: Data-driven 6D Pose Tracking by Calibrating Image Residuals in Synthetic Domains}},
booktitle = {IEEE/RSJ International Conference on Intelligent Robots and Systems (IROS)},
}

@inproceedings{Wuthrich_Tracking_2013_IROS,
author = {Wuthrich, Manuel and Pastor, Peter and Kalakrishnan, Mrinal and Bohg, Jeannette and Schaal, Stefan},
year = {2013},
month = {11},
pages = {3195-3202},
title = {Probabilistic Object Tracking using a Range Camera},
booktitle = {IEEE/RSJ International Conference on Intelligent Robots and Systems (IROS)},
doi = {10.1109/IROS.2013.6696810}
}

@inproceedings{Choi_Pose_Tracking_2013_IROS,
author = {Choi, Changhyun and Christensen, Henrik},
year = {2013},
month = {11},
pages = {1084-1091},
title = {{RGB-D object tracking: A particle filter approach on GPU}},
booktitle = {IEEE/RSJ International Conference on Intelligent Robots and Systems (IROS)},
doi = {10.1109/IROS.2013.6696485}
}

@inproceedings{Choi_Textureless_2012_IROS,
author = {Choi, Changhyun and Christensen, Henrik},
year = {2012},
month = {10},
pages = {},
title = {3D Textureless Object Detection and Tracking: An Edge-based approach},
journal = {IEEE International Conference on Intelligent Robots and Systems},
doi = {10.1109/IROS.2012.6386065}
}

@inproceedings{Dart_2014_RSS,
author = {Schmidt, Tanner and Newcombe, Richard and Fox, Dieter},
year = {2014},
month = {07},
pages = {},
title = {{DART: Dense Articulated Real-Time Tracking}},
doi = {10.15607/RSS.2014.X.030},
BOOKTITLE = {Proceedings of Robotics: Science and Systems},
}

@inproceedings{SimTrack_2015_IROS,
author = {Pauwels, Karl and Kragic, Danica},
year = {2015},
month = {09},
pages = {1300-1307},
title = {SimTrack: A simulation-based framework for scalable real-time object pose detection and tracking},
doi = {10.1109/IROS.2015.7353536}
}

@inproceedings{Multi_Forest_Tracker_CVPR_2014,
author = {Tan, David Joseph and Ilic, Slobodan},
year = {2014},
month = {06},
pages = {},
title = {{Multi-Forest Tracker: A Chameleon in Tracking}},
booktitle = {IEEE Conference on Computer Vision and Pattern Recognition (CVPR)},
doi = {10.1109/CVPR.2014.157}
}
@inproceedings{3D_Temporal_Tracker_ICCV_2015,
author = {Tan, David Joseph and Tombari, Federico and Ilic, Slobodan and Navab, Nassir},
year = {2015},
month = {12},
pages = {693-701},
title = {{A Versatile Learning-Based 3D Temporal Tracker: Scalable, Robust, Online}},
doi = {10.1109/ICCV.2015.86},
booktitle = {IEEE International Conference on Computer Vision (ICCV)}
}

@article{6_DOF_Tracking_2017_TVCG,
author = {Garon, Mathieu and Lalonde, Jean-François},
year = {2017},
month = {03},
pages = {},
title = {{Deep 6-DOF Tracking}},
volume = {PP},
journal = {IEEE Transactions on Visualization and Computer Graphics},
doi = {10.1109/TVCG.2017.2734599}
}

@inproceedings{Manhardt_ICCV_2019,
author = {Manhardt, Fabian and Arroyo, Diego and Rupprecht, Christian and Busam, Benjamin and Navab, Nassir and Tombari, Federico},
year = {2018},
month = {12},
pages = {},
title = {{Explaining the Ambiguity of Object Detection and 6D Pose from Visual Data}},
booktitle = {IEEE International Conference on Computer Vision (ICCV)}
}

@article{Textureless_Hinterstoisser_2012_TPAMI,
author = {Hinterstoisser, Stefan and Cagniart, Cedric and Ilic, Slobodan and Sturm, Peter and Navab, Nassir and Fua, Pascal and Lepetit, Vincent and Lepetit, bullet},
year = {2012},
month = {05},
pages = {},
title = {{Gradient Response Maps for Real-Time Detection of Texture-Less Objects}},
volume = {1},
journal = {IEEE TRANSACTIONS ON PATTERN ANALYSIS AND MACHINE INTELLIGENCE (TPAMI)},
doi = {10.1109/TPAMI.2011.206}
}

@inproceedings{Seg_Gupta_2015_CVPR,
author = {Gupta, Saurabh and Arbelaez, Pablo and Girshick, Ross and Malik, Jitendra},
year = {2015},
month = {06},
pages = {4731-4740},
title = {Aligning 3D models to RGB-D images of cluttered scenes},
booktitle = {The IEEE Conference on Computer Vision and Pattern Recognition (CVPR)},
doi = {10.1109/CVPR.2015.7299105}
}

@inproceedings{Textureless_Wohlhart_2015_CVPR,
author = {Wohlhart, Paul and Lepetit, Vincent},
year = {2015},
month = {06},
pages = {3109-3118},
title = {Learning descriptors for object recognition and 3D pose estimation},
booktitle = {The IEEE Conference on Computer Vision and Pattern Recognition (CVPR)},
doi = {10.1109/CVPR.2015.7298930}
}

@inproceedings{Textureless_2016_ICRA,
author = {Cao, Zhe and Sheikh, Yaser and Banerjee, Natasha},
year = {2016},
month = {05},
pages = {2441-2448},
title = {Real-time scalable 6DOF pose estimation for textureless objects},
doi = {10.1109/ICRA.2016.7487396}
}

@article{Rotation_Avarage,
author = {Moakher, Maher},
year = {2002},
month = {04},
pages = {},
title = {Means and Averaging in the Group of Rotations},
volume = {24},
journal = {SIAM Journal on Matrix Analysis and Applications},
doi = {10.1137/S0895479801383877}
}

@InProceedings{Vovel_Space_Method_2016_CVPR,
author = {Song, Shuran and Xiao, Jianxiong},
title = {Deep Sliding Shapes for Amodal 3D Object Detection in RGB-D Images},
booktitle = {The IEEE Conference on Computer Vision and Pattern Recognition (CVPR)},
month = {June},
year = {2016}
}

@InProceedings{Frustum_Pointnet_2018_CVPR,
author = {Qi, Charles R. and Liu, Wei and Wu, Chenxia and Su, Hao and Guibas, Leonidas J.},
title = {Frustum PointNets for 3D Object Detection From RGB-D Data},
booktitle = {The IEEE Conference on Computer Vision and Pattern Recognition (CVPR)},
month = {June},
year = {2018}
}
@InProceedings{RGB_D_Directly_2018_ECCV,
author = {Li, Chi and Bai, Jin and Hager, Gregory D.},
title = {A Unified Framework for Multi-View Multi-Class Object Pose Estimation},
booktitle = {The European Conference on Computer Vision (ECCV)},
month = {September},
year = {2018}
}

@InProceedings{Pointnet_2017_CVPR,
author = {Qi, Charles R. and Su, Hao and Mo, Kaichun and Guibas, Leonidas J.},
title = {PointNet: Deep Learning on Point Sets for 3D Classification and Segmentation},
booktitle = {The IEEE Conference on Computer Vision and Pattern Recognition (CVPR)},
month = {July},
year = {2017}
}

@conference{YCB_Dataset,
author = {Berk Calli and Arjun Singh and Aaron Walsman and Siddhartha Srinivasa and Pieter Abbeel and Aaron Dollar},
title = {{The YCB Object and Model Set: Towards Common Benchmarks for Manipulation Research}},
booktitle = {Proceedings of IEEE International Conference on Advanced Robotics (ICAR)},
year = {2015},
month = {July}
}

@InProceedings{PVNet,
author = {Peng, Sida and Liu, Yuan and Huang, Qixing and Zhou, Xiaowei and Bao, Hujun},
title = {{PVNet: Pixel-Wise Voting Network for 6DoF Pose Estimation}},
booktitle = {IEEE Conference on Computer Vision and Pattern Recognition (CVPR)},
month = {June},
year = {2019}
}
@InProceedings{SSD_ECCV_2016,
author="Liu, Wei
and Anguelov, Dragomir
and Erhan, Dumitru
and Szegedy, Christian
and Reed, Scott
and Fu, Cheng-Yang
and Berg, Alexander C.",
title= {{SSD: Single Shot MultiBox Detector}},
booktitle="Proceedings of the European Conference on Computer Vision (ECCV)",
year="2016",
pages="21--37",
isbn="978-3-319-46448-0"
}

@InProceedings{Classif_2_2015_ICCV,
author = {Su, Hao and Qi, Charles R. and Li, Yangyan and Guibas, Leonidas J.},
title = {Render for CNN: Viewpoint Estimation in Images Using CNNs Trained With Rendered 3D Model Views},
booktitle = {IEEE International Conference on Computer Vision (ICCV)},
month = {December},
year = {2015}
}

@InProceedings{Symmtry_Oberweger_2018_ECCV,
author = {Oberweger, Markus and Rad, Mahdi and Lepetit, Vincent},
title = {{Making Deep Heatmaps Robust to Partial Occlusions for 3D Object Pose Estimation}},
booktitle = {Proceedings of the European Conference on Computer Vision (ECCV)},
month = {September},
year = {2018}
}

@InProceedings{BB8_Rad_2017_ICCV,
author = {Rad, Mahdi and Lepetit, Vincent},
title = {{BB8: A Scalable, Accurate, Robust to Partial Occlusion Method for Predicting the 3D Poses of Challenging Objects Without Using Depth}},
booktitle = {IEEE International Conference on Computer Vision (ICCV)},
month = {Oct},
year = {2017}
}


@inproceedings{SSD_6D_ICCV_2017,
author = {Kehl, Wadim and Manhardt, Fabian and Tombari, Federico and Ilic, Slobodan and Navab, Nassir},
year = {2017},
month = {10},
pages = {1530-1538},
title = {{SSD-6D: Making RGB-Based 3D Detection and 6D Pose Estimation Great Again}},
doi = {10.1109/ICCV.2017.169},
booktitle = {IEEE International Conference on Computer Vision (ICCV)},
}

@INPROCEEDINGS{Symmetry_Pitteri_2019_3DV,
  author={G. {Pitteri} and M. {Ramamonjisoa} and S. {Ilic} and V. {Lepetit}},
  booktitle={International Conference on 3D Vision (3DV)}, 
  title={{On Object Symmetries and 6D Pose Estimation from Images}}, 
  year={2019},
  volume={},
  number={},
  pages={614-622},}


@article{VGG_2014,
author = {Simonyan, Karen and Zisserman, Andrew},
year = {2014},
month = {09},
pages = {},
title = {Very Deep Convolutional Networks for Large-Scale Image Recognition},
journal = {arXiv 1409.1556}
}

@InProceedings{Classfi_3_2018_ECCV,
author = {Sundermeyer, Martin and Marton, Zoltan-Csaba and Durner, Maximilian and Brucker, Manuel and Triebel, Rudolph},
title = {Implicit 3D Orientation Learning for 6D Object Detection from RGB Images},
booktitle = {The European Conference on Computer Vision (ECCV)},
month = {September},
year = {2018}
}

@InProceedings{SURF,
author="Bay, Herbert
and Tuytelaars, Tinne
and Van Gool, Luc",
editor="Leonardis, Ale{\v{s}}
and Bischof, Horst
and Pinz, Axel",
title="SURF: Speeded Up Robust Features",
booktitle="Computer Vision -- ECCV 2006",
year="2006",
publisher="Springer Berlin Heidelberg",
address="Berlin, Heidelberg",
pages="404--417",
abstract="In this paper, we present a novel scale- and rotation-invariant interest point detector and descriptor, coined SURF (Speeded Up Robust Features). It approximates or even outperforms previously proposed schemes with respect to repeatability, distinctiveness, and robustness, yet can be computed and compared much faster.",
isbn="978-3-540-33833-8"
}

@INPROCEEDINGS{Tradit_ICCV_1999, 
author={D. G. {Lowe}}, 
booktitle={Proceedings of the Seventh IEEE International Conference on Computer Vision}, 
title={Object recognition from local scale-invariant features}, 
year={1999}, 
volume={2}, 
number={}, 
pages={1150-1157 vol.2}, 
doi={10.1109/ICCV.1999.790410}, 
ISSN={null}, 
month={Sep.},}

@article{Tradit_1_IJCV_2006,
author = {Rothganger, Fred and Lazebnik, Svetlana and Schmid, Cordelia and Ponce, J.},
year = {2006},
month = {03},
pages = {231-259},
title = {3D Object Modeling and Recognition Using Local Affine-Invariant Image Descriptors and Multi-View Spatial Constraints},
volume = {66},
journal = {International Journal of Computer Vision},
doi = {10.1007/s11263-005-3674-1}
}

@InProceedings{HeatMap_1_2018_ECCV,
author = {Oberweger, Markus and Rad, Mahdi and Lepetit, Vincent},
title = {Making Deep Heatmaps Robust to Partial Occlusions for 3D Object Pose Estimation},
booktitle = {The European Conference on Computer Vision (ECCV)},
month = {September},
year = {2018}
}

@INPROCEEDINGS{HeatMap_2_ICRA_2017, 
author={G. {Pavlakos} and X. {Zhou} and A. {Chan} and K. G. {Derpanis} and K. {Daniilidis}}, 
booktitle={2017 IEEE International Conference on Robotics and Automation (ICRA)}, 
title={6-DoF object pose from semantic keypoints}, 
year={2017}, 
volume={}, 
number={}, 
pages={2011-2018}, 
doi={10.1109/ICRA.2017.7989233}, 
ISSN={null}, 
month={May},}


@InProceedings{Pixelwise_3D_Point_2017_CVPR,
author = {Michel, Frank and Kirillov, Alexander and Brachmann, Eric and Krull, Alexander and Gumhold, Stefan and Savchynskyy, Bogdan and Rother, Carsten},
title = {Global Hypothesis Generation for 6D Object Pose Estimation},
booktitle = {The IEEE Conference on Computer Vision and Pattern Recognition (CVPR)},
month = {July},
year = {2017}
}
@misc{Hybridpose_2020,
    title={HybridPose: 6D Object Pose Estimation under Hybrid Representations},
    author={Chen Song and Jiaru Song and Qixing Huang},
    year={2020},
    eprint={2001.01869},
    archivePrefix={arXiv},
    primaryClass={cs.CV}
}

@article{EPnP,
author = {Lepetit, Vincent and Moreno-Noguer, Francesc and Fua, Pascal},
year = {2009},
month = {02},
pages = {},
title = {{EPnP: An accurate O(n) solution to the PnP problem}},
volume = {81},
journal = {International Journal of Computer Vision (IJCV)},
doi = {10.1007/s11263-008-0152-6}
}

@INPROCEEDINGS{Sun397, 
author={J. {Xiao} and J. {Hays} and K. A. {Ehinger} and A. {Oliva} and A. {Torralba}}, 
booktitle={2010 IEEE Computer Society Conference on Computer Vision and Pattern Recognition}, 
title={SUN database: Large-scale scene recognition from abbey to zoo}, 
year={2010}, 
volume={}, 
number={}, 
pages={3485-3492}, 
doi={10.1109/CVPR.2010.5539970}, 
ISSN={1063-6919}, 
month={June},
}


@article{Maskrcnn_2017,
  author    = {Kaiming He and
               Georgia Gkioxari and
               Piotr Doll{\'{a}}r and
               Ross B. Girshick},
  title     = {Mask {R-CNN}},
  journal   = {CoRR},
  volume    = {abs/1703.06870},
  year      = {2017},
  url       = {http://arxiv.org/abs/1703.06870},
  eprinttype = {arXiv},
  eprint    = {1703.06870},
  timestamp = {Mon, 13 Aug 2018 16:46:36 +0200},
  biburl    = {https://dblp.org/rec/journals/corr/HeGDG17.bib},
  bibsource = {dblp computer science bibliography, https://dblp.org}
}

@misc{Shapenet_2015,
  abstract = { },
  added-at = {2018-04-27T07:45:00.000+0200},
  author = {Chang, Angel X. and Funkhouser, Thomas and Guibas, Leonidas and Hanrahan, Pat and Huang, Qixing and Li, Zimo and Savarese, Silvio and Savva, Manolis and Song, Shuran and Su, Hao and Xiao, Jianxiong and Yi, Li and Yu, Fisher},
  biburl = {https://www.bibsonomy.org/bibtex/247acee8c2cc6c465b98fc499711dd6c3/achakraborty},
  description = {[1512.03012] ShapeNet: An Information-Rich 3D Model Repository},
  interhash = {44fc945ba9bb97661d706e2afb0a9c4d},
  intrahash = {47acee8c2cc6c465b98fc499711dd6c3},
  keywords = {2015 3D data dataset shape},
  note = {cite arxiv:1512.03012},
  timestamp = {2018-04-27T07:45:00.000+0200},
  title = {ShapeNet: An Information-Rich 3D Model Repository},
  url = {http://arxiv.org/abs/1512.03012},
  year = 2015
}

@INPROCEEDINGS{DensePose_2018_CVPR, 
author={R. A. {Güler} and N. {Neverova} and I. {Kokkinos}}, 
booktitle={2018 IEEE/CVF Conference on Computer Vision and Pattern Recognition}, 
title={DensePose: Dense Human Pose Estimation in the Wild}, 
year={2018}, 
volume={}, 
number={}, 
pages={7297-7306}, 
keywords={convolutional neural nets;pose estimation;dense human pose estimation;surface-based representation;human body;COCO dataset;CNN-based systems;fully-convolutional networks;region-based models;Pose estimation;Three-dimensional displays;Task analysis;Solid modeling;Training;Pipelines;Deformable models}, 
doi={10.1109/CVPR.2018.00762}, 
ISSN={1063-6919}, 
month={June},}


@INPROCEEDINGS{Camera_Relocalization_1, 
author={J. {Shotton} and B. {Glocker} and C. {Zach} and S. {Izadi} and A. {Criminisi} and A. {Fitzgibbon}}, 
booktitle={2013 IEEE Conference on Computer Vision and Pattern Recognition}, 
title={Scene Coordinate Regression Forests for Camera Relocalization in RGB-D Images}, 
year={2013}, 
volume={}, 
number={}, 
pages={2930-2937}, 
doi={10.1109/CVPR.2013.377}, 
ISSN={1063-6919}, 
month={June},}


@INPROCEEDINGS{Camera_Relocalization_2, 
author={J. {Valentin} and M. {Nießner} and J. {Shotton} and A. {Fitzgibbon} and S. {Izadi} and P. {Torr}}, 
booktitle={2015 IEEE Conference on Computer Vision and Pattern Recognition (CVPR)}, 
title={Exploiting uncertainty in regression forests for accurate camera relocalization}, 
year={2015}, 
volume={}, 
number={}, 
pages={4400-4408}, 
doi={10.1109/CVPR.2015.7299069}, 
ISSN={1063-6919}, 
month={June},}


@ARTICLE{Umeyama, 
author={S. {Umeyama}}, 
journal={IEEE Transactions on Pattern Analysis and Machine Intelligence}, 
title={Least-squares estimation of transformation parameters between two point patterns}, 
year={1991}, 
volume={13}, 
number={4}, 
pages={376-380}, 
doi={10.1109/34.88573}, 
ISSN={1939-3539}, 
month={April},}
}

@unknown{Single_Stage_2020_CVPR,
author = {Hu, Yinlin and Fua, Pascal and Wang, Wei and Salzmann, Mathieu},
year = {2019},
month = {11},
pages = {},
title = {{Single-Stage 6D Object Pose Estimation}},
booktitle = {IEEE Conference on Computer Vision and Pattern Recognition (CVPR)}
}

@InProceedings{Seg_Driven_2019_CVPR,
author = {Hu, Yinlin and Hugonot, Joachim and Fua, Pascal and Salzmann, Mathieu},
title = {{Segmentation-Driven 6D Object Pose Estimation}},
booktitle = {IEEE Conference on Computer Vision and Pattern Recognition (CVPR)},
month = {June},
year = {2019}
}

@misc{YOLOv3,
  added-at = {2018-09-21T15:24:42.000+0200},
  author = {Redmon, Joseph and Farhadi, Ali},
  biburl = {https://www.bibsonomy.org/bibtex/2cd221fb00896b020dec735d19ff2d9bd/tgandor},
  description = {YOLOv3: An Incremental Improvement},
  interhash = {bbdec3df168e9809d9e61423d4b4e062},
  intrahash = {cd221fb00896b020dec735d19ff2d9bd},
  keywords = {cnn deep_learning object_detection yolo},
  note = {cite arxiv:1804.02767Comment: Tech Report},
  timestamp = {2018-09-21T15:24:42.000+0200},
  title = {YOLOv3: An Incremental Improvement},
  url = {http://arxiv.org/abs/1804.02767},
  year = 2018
}

@InProceedings{FocalLoss_2017_ICCV,
author = {Lin, Tsung-Yi and Goyal, Priya and Girshick, Ross and He, Kaiming and Dollar, Piotr},
title = {Focal Loss for Dense Object Detection},
booktitle = {The IEEE International Conference on Computer Vision (ICCV)},
month = {Oct},
year = {2017}
}

@inproceedings{DOT_Hinterstoisser_2010_CVPR,
author = {Hinterstoisser, Stefan and Lepetit, Vincent and Ilic, Slobodan and Fua, Pascal and Navab, Nassir},
year = {2010},
month = {09},
pages = {2257-2264},
title = {{Dominant Orientation Templates for Real-Time Detection of Texture-Less Objects}},
booktitle = {IEEE Conference on Computer Vision and Pattern Recognition (CVPR)},
doi = {10.1109/CVPR.2010.5539908}
}

@ARTICLE{SegNet, 
author={V. {Badrinarayanan} and A. {Kendall} and R. {Cipolla}}, 
journal={IEEE Transactions on Pattern Analysis and Machine Intelligence}, 
title={SegNet: A Deep Convolutional Encoder-Decoder Architecture for Image Segmentation}, 
year={2017}, 
volume={39}, 
number={12}, 
pages={2481-2495}, 
doi={10.1109/TPAMI.2016.2644615}, 
ISSN={1939-3539}, 
month={Dec},}
}

@article{Random_Erasing,
author = {Zhong, Zhun and Zheng, Liang and Kang, Guoliang and Li, Shaozi and Yang, Yi},
year = {2017},
month = {08},
pages = {},
title = {Random Erasing Data Augmentation}
}

@ARTICLE{Hausdorff, 
author={D. P. {Huttenlocher} and G. A. {Klanderman} and W. J. {Rucklidge}}, 
journal={IEEE Transactions on Pattern Analysis and Machine Intelligence}, 
title={Comparing images using the Hausdorff distance}, 
year={1993}, 
volume={15}, 
number={9}, 
pages={850-863}, 
keywords={image processing;image comparison;translation;position error tolerance;Hausdorff distance;binary image;rigid motion;shape comparison methods;Shape;Image edge detection;Pattern recognition;Detectors;Feature extraction;Computer vision;Pattern matching;Councils;Scholarships;Computer science}, 
doi={10.1109/34.232073}, 
ISSN={1939-3539}, 
month={Sep.}
}
@INPROCEEDINGS{Chamfer, 
author={M. {Liu} and O. {Tuzel} and A. {Veeraraghavan} and R. {Chellappa}}, 
booktitle={2010 IEEE Computer Society Conference on Computer Vision and Pattern Recognition}, 
title={Fast directional chamfer matching}, 
year={2010}, 
volume={}, 
number={}, 
pages={1696-1703}, 
doi={10.1109/CVPR.2010.5539837}, 
ISSN={1063-6919}, 
month={June}
}

@inproceedings{Rios-Cabrera_discriminative,
author = {Rios-Cabrera, Reyes and Tuytelaars, Tinne},
year = {2013},
month = {12},
pages = {2048-2055},
title = {{Discriminatively Trained Templates for 3D Object Detection: A Real Time Scalable Approach}},
booktitle = {IEEE International Conference on Computer Vision (ICCV)},
doi = {10.1109/ICCV.2013.256}
}

@inproceedings{Cai_Textureless_2013_CVS,
author = {Cai, Hongping and Werner, Tomas and Matas, Jiri},
year = {2013},
month = {07},
pages = {103-112},
title = {{Fast Detection of Multiple Textureless 3-D Objects}},
booktitle={Computer Vision Systems},
doi = {10.1007/978-3-642-39402-7_11}
}

@InProceedings{CDPN,
author = {Li, Zhigang and Wang, Gu and Ji, Xiangyang},
title = {CDPN: Coordinates-Based Disentangled Pose Network for Real-Time RGB-Based 6-DoF Object Pose Estimation},
booktitle = {The IEEE International Conference on Computer Vision (ICCV)},
month = {October},
year = {2019}
}

@InProceedings{Pix2Pose_2019_ICCV,
author = {Park, Kiru and Patten, Timothy and Vincze, Markus},
title = {{Pix2Pose: Pixel-Wise Coordinate Regression of Objects for 6D Pose Estimation}},
booktitle = {IEEE International Conference on Computer Vision (ICCV)},
month = {October},
year = {2019}
}

@InProceedings{DPOD_2019_ICCV,
author = {Zakharov, Sergey and Shugurov, Ivan and Ilic, Slobodan},
title = {{DPOD: 6D Pose Object Detector and Refiner}},
booktitle = {The IEEE International Conference on Computer Vision (ICCV)},
month = {October},
year = {2019}
}

@InProceedings{DeepIM_2018_ECCV,
author = {Li, Yi and Wang, Gu and Ji, Xiangyang and Xiang, Yu and Fox, Dieter},
title = {DeepIM: Deep Iterative Matching for 6D Pose Estimation},
booktitle = {Proceedings of the European Conference on Computer Vision (ECCV)},
month = {September},
year = {2018}
} 

@unknown{Articulated_Pose,
author = {Li, Xiaolong and Wang, He and Yi, Li and Guibas, Leonidas and Abbott, A. and Song, Shuran},
year = {2019},
month = {12},
pages = {},
title = {Category-Level Articulated Object Pose Estimation}
}
@InProceedings{Limitaion_2019_CVPR,
author = {Sattler, Torsten and Zhou, Qunjie and Pollefeys, Marc and Leal-Taixe, Laura},
title = {Understanding the Limitations of CNN-Based Absolute Camera Pose Regression},
booktitle = {The IEEE Conference on Computer Vision and Pattern Recognition (CVPR)},
month = {June},
year = {2019}
}

@unknown{CullNet,
author = {Gupta, Kartik and Petersson, Lars and Hartley, Richard},
year = {2019},
month = {09},
pages = {},
title = {CullNet: Calibrated and Pose Aware Confidence Scores for Object Pose Estimation}
}
@inproceedings{IC_MI_Dataset,
author = {Tejani, Alykhan and Tang, Danhang and Kouskouridas, Rigas and Kim, Tae-Kyun},
year = {2014},
month = {09},
pages = {462-477},
title = {Latent-Class Hough Forests for 3D Object Detection and Pose Estimation},
doi = {10.1007/978-3-319-10599-4_30}
}
@inproceedings{IC_BIN_Dataset,
author = {Doumanoglou, Andreas and Kouskouridas, Rigas and Malassiotis, Sotiris and Kim, Tae-Kyun},
year = {2016},
month = {06},
pages = {3583-3592},
title = {Recovering 6D Object Pose and Predicting Next-Best-View in the Crowd},
doi = {10.1109/CVPR.2016.390}
}
@article{RU_APC_Dataset,
author = {Rennie, Colin and Shome, Rahul and Bekris, Kostas and De Souza, Alberto},
year = {2015},
month = {09},
pages = {},
title = {A Dataset for Improved RGBD-Based Object Detection and Pose Estimation for Warehouse Pick-and-Place},
volume = {1},
journal = {IEEE Robotics and Automation Letters},
doi = {10.1109/LRA.2016.2532924}
}

@article{Amazon_Picking_Challenge,
author = {Correll, Nikolaus and Bekris, Kostas and Berenson, Dmitry and Brock, Oliver and Causo, Albert and Hauser, Kris and Okada, Kei and Rodríguez, Alberto and Romano, Joseph and Wurman, Peter},
year = {2016},
month = {01},
pages = {},
title = {Lessons from the Amazon Picking Challenge}
}

@inproceedings{Roberto2014ArticulatedIROS,
author = {Martin-Martin, Roberto and Brock, Oliver},
year = {2014},
month = {09},
pages = {},
title = {Online interactive perception of articulated objects with multi-level recursive estimation based on task-specific priors},
journal = {IEEE International Conference on Intelligent Robots and Systems},
doi = {10.1109/IROS.2014.6942902}
}

@inproceedings{Roberto2016ArticulatedICRA,
author = {Martin-Martin, Roberto and Höfer, Sebastian and Brock, Oliver},
year = {2016},
month = {05},
pages = {},
title = {An Integrated Approach to Visual Perception of Articulated Objects},
doi = {10.1109/ICRA.2016.7487714}
}

@inproceedings{Katz2013InteractiveArticulatedICRA,
author = {Katz, Dov and Kazemi, Moslem and Bagnell, J. and Stentz, Anthony},
year = {2013},
month = {05},
pages = {5003-5010},
title = {Interactive segmentation, tracking, and kinematic modeling of unknown 3D articulated objects},
isbn = {978-1-4673-5641-1},
journal = {Proceedings - IEEE International Conference on Robotics and Automation},
doi = {10.1109/ICRA.2013.6631292}
}

@inproceedings{3D_RCNN_2018KunduCVPR,
author = {Kundu, Abhijit and Li, Yin and Rehg, James},
year = {2018},
month = {06},
pages = {3559-3568},
title = {3D-RCNN: Instance-Level 3D Object Reconstruction via Render-and-Compare},
doi = {10.1109/CVPR.2018.00375}
}

@article{DeepIM_IJCV_Version_Li_2020,
author = {Li, Yi and Wang, Gu and Ji, Xiangyang and Xiang, Yu and Fox, Dieter},
year = {2020},
month = {03},
pages = {},
title = {DeepIM: Deep Iterative Matching for 6D Pose Estimation},
volume = {128},
journal = {International Journal of Computer Vision},
doi = {10.1007/s11263-019-01250-9}
}

@article{wang2019_6_pack,
  title={6-PACK: Category-level 6D Pose Tracker with Anchor-Based Keypoints},
  author={Wang, Chen and Mart{\'\i}n-Mart{\'\i}n, Roberto and Xu, Danfei and Lv, Jun and Lu, Cewu and Fei-Fei, Li and Savarese, Silvio and Zhu, Yuke},
  booktitle={International Conference on Robotics and Automation (ICRA)},
  year={2020}
}

@inproceedings{CDBT_2D_Tracking_Benchmark_2019_ICCV,
author = {Lukežič, Alan and Kart, Ugur and Kapyla, Jani and Durmush, Ahmed and Kamarainen, Joni-Kristian and Matas, Jiri and Kristan, Matej},
year = {2019},
month = {10},
pages = {10012-10021},
title = {CDTB: A Color and Depth Visual Object Tracking Dataset and Benchmark},
doi = {10.1109/ICCV.2019.01011}
}

@INPROCEEDINGS{Roy_2D_Tracking_Benchmark_2015_ICRA,  
author={A. {Roy} and  {Xi Zhang} and N. {Wolleb} and C. P. {Quintero} and M. {Jägersand}},  
booktitle={2015 IEEE International Conference on Robotics and Automation (ICRA)},   
title={Tracking benchmark and evaluation for manipulation tasks},   
year={2015},  
volume={},  
number={},  
pages={2448-2453},  
doi={10.1109/ICRA.2015.7139526}}

@inproceedings{HumenPose_Tracking_Benchmark,
author = {Andriluka, Mykhaylo and Iqbal, Umar and Insafutdinov, Eldar and Pishchulin, Leonid and Milan, Anton and Gall, Juergen and Schiele, Bernt},
year = {2018},
month = {06},
pages = {5167-5176},
title = {PoseTrack: A Benchmark for Human Pose Estimation and Tracking},
doi = {10.1109/CVPR.2018.00542}
}

@InProceedings{Kart_2019_CVPR_2D_Tracking,
author = {Kart, Ugur and Lukezic, Alan and Kristan, Matej and Kamarainen, Joni-Kristian and Matas, Jiri},
title = {Object Tracking by Reconstruction With View-Specific Discriminative Correlation Filters},
booktitle = {Proceedings of the IEEE/CVF Conference on Computer Vision and Pattern Recognition (CVPR)},
month = {June},
year = {2019}
}

@INPROCEEDINGS{TUW_dataset_2015,  
author={T. {Fäulhammer} and A. {Aldoma} and M. {Zillich} and M. {Vincze}},  
booktitle={2015 IEEE International Conference on Robotics and Automation (ICRA)},   
title={Temporal integration of feature correspondences for enhanced recognition in cluttered and dynamic environments},   
year={2015},  
volume={},  
number={},  
pages={3003-3009},  
doi={10.1109/ICRA.2015.7139611}}

@INPROCEEDINGS{UW_RGBD_Dataset_2011_ICRA,
  author={K. {Lai} and L. {Bo} and X. {Ren} and D. {Fox}},
  booktitle={2011 IEEE International Conference on Robotics and Automation}, 
  title={A large-scale hierarchical multi-view RGB-D object dataset}, 
  year={2011},
  volume={},
  number={},
  pages={1817-1824},
  doi={10.1109/ICRA.2011.5980382}}

@InProceedings{DAKDN_2021_CVPR,
    author    = {Zhang, Shaobo and Zhao, Wanqing and Guan, Ziyu and Peng, Xianlin and Peng, Jinye},
    title     = {Keypoint-Graph-Driven Learning Framework for Object Pose Estimation},
    booktitle = {Proceedings of the IEEE/CVF Conference on Computer Vision and Pattern Recognition (CVPR)},
    month     = {June},
    year      = {2021},
    pages     = {1065-1073}
}

@article{kpam_2019,
  author    = {Lucas Manuelli and
               Wei Gao and
               Peter R. Florence and
               Russ Tedrake},
  title     = {kPAM: KeyPoint Affordances for Category-Level Robotic Manipulation},
  journal   = {CoRR},
  volume    = {abs/1903.06684},
  year      = {2019},
  url       = {http://arxiv.org/abs/1903.06684},
  eprinttype = {arXiv},
  eprint    = {1903.06684},
  timestamp = {Mon, 01 Apr 2019 14:07:37 +0200},
  biburl    = {https://dblp.org/rec/journals/corr/abs-1903-06684.bib},
  bibsource = {dblp computer science bibliography, https://dblp.org}
}



@article{kpam2_2021_RSS,
  author    = {Wei Gao and
               Russ Tedrake},
  title     = {kPAM 2.0: Feedback Control for Category-Level Robotic Manipulation},
  journal   = {CoRR},
  volume    = {abs/2102.06279},
  year      = {2021},
  url       = {https://arxiv.org/abs/2102.06279},
  eprinttype = {arXiv},
  eprint    = {2102.06279},
  timestamp = {Thu, 18 Feb 2021 15:26:00 +0100},
  biburl    = {https://dblp.org/rec/journals/corr/abs-2102-06279.bib},
  bibsource = {dblp computer science bibliography, https://dblp.org}
}



@article{MLP_Mixer_2021,
  author    = {Ilya O. Tolstikhin and
               Neil Houlsby and
               Alexander Kolesnikov and
               Lucas Beyer and
               Xiaohua Zhai and
               Thomas Unterthiner and
               Jessica Yung and
               Andreas Steiner and
               Daniel Keysers and
               Jakob Uszkoreit and
               Mario Lucic and
               Alexey Dosovitskiy},
  title     = {MLP-Mixer: An all-MLP Architecture for Vision},
  journal   = {CoRR},
  volume    = {abs/2105.01601},
  year      = {2021},
  url       = {https://arxiv.org/abs/2105.01601},
  eprinttype = {arXiv},
  eprint    = {2105.01601},
  timestamp = {Tue, 18 May 2021 10:37:34 +0200},
  biburl    = {https://dblp.org/rec/journals/corr/abs-2105-01601.bib},
  bibsource = {dblp computer science bibliography, https://dblp.org}
}


@article{DONet_Lin_2021,
  title={DONet: Learning Category-Level 6D Object Pose and Size Estimation from Depth Observation},
  author={Haitao Lin and Zichang Liu and Chi-Hou Cheang and Lingwei Zhang and Yanwei Fu and X. Xue},
  journal={ArXiv},
  year={2021},
  volume={abs/2106.14193}
}

@misc{GPV-Pose_2022_CVPR,
  doi = {10.48550/ARXIV.2203.07918},
  
  url = {https://arxiv.org/abs/2203.07918},
  
  author = {Di, Yan and Zhang, Ruida and Lou, Zhiqiang and Manhardt, Fabian and Ji, Xiangyang and Navab, Nassir and Tombari, Federico},
  
  keywords = {Computer Vision and Pattern Recognition (cs.CV), FOS: Computer and information sciences, FOS: Computer and information sciences},
  
  title = {GPV-Pose: Category-level Object Pose Estimation via Geometry-guided Point-wise Voting},
  
  publisher = {arXiv},
  
  year = {2022},
  
  copyright = {Creative Commons Attribution Non Commercial Share Alike 4.0 International}
}

@inproceedings{GPV-Pose_2022_CVPR_reb,
  doi = {10.48550/ARXIV.2203.07918},
  
  url = {https://arxiv.org/abs/2203.07918},
  
  author = {Di et al.},
  
  keywords = {Computer Vision and Pattern Recognition (cs.CV), FOS: Computer and information sciences, FOS: Computer and information sciences},
  
  title = {{GPV-Pose}: Category-level Object Pose Estimation via Geometry-guided Point-wise Voting},
  
  publisher = {CVPR},
  
  year = {2022},
  
  copyright = {Creative Commons Attribution Non Commercial Share Alike 4.0 International}
}

@software{YOLOv5_2020,
  author       = {Glenn Jocher and
                  Ayush Chaurasia and
                  Alex Stoken and
                  Jirka Borovec and
                  NanoCode012 and
                  Yonghye Kwon and
                  TaoXie and
                  Jiacong Fang and
                  imyhxy and
                  Kalen Michael and
                  Lorna and
                  Abhiram V and
                  Diego Montes and
                  Jebastin Nadar and
                  Laughing and
                  tkianai and
                  yxNONG and
                  Piotr Skalski and
                  Zhiqiang Wang and
                  Adam Hogan and
                  Cristi Fati and
                  Lorenzo Mammana and
                  AlexWang1900 and
                  Deep Patel and
                  Ding Yiwei and
                  Felix You and
                  Jan Hajek and
                  Laurentiu Diaconu and
                  Mai Thanh Minh},
  title        = {{ultralytics/yolov5: v6.1 - TensorRT, TensorFlow 
                   Edge TPU and OpenVINO Export and Inference}},
  month        = feb,
  year         = 2022,
  publisher    = {Zenodo},
  version      = {v6.1},
  doi          = {10.5281/zenodo.6222936},
  url          = {https://doi.org/10.5281/zenodo.6222936}
}


@InProceedings{DualPoseNet_2021_ICCV,
    author    = {Lin, Jiehong and Wei, Zewei and Li, Zhihao and Xu, Songcen and Jia, Kui and Li, Yuanqing},
    title     = {DualPoseNet: Category-Level 6D Object Pose and Size Estimation Using Dual Pose Network With Refined Learning of Pose Consistency},
    booktitle = {Proceedings of the IEEE/CVF International Conference on Computer Vision (ICCV)},
    month     = {October},
    year      = {2021},
    pages     = {3560-3569}
}

@inproceedings{CR-Net_2021_IROS,
  title={Category-level 6d object pose estimation via cascaded relation and recurrent reconstruction networks},
  author={Wang, Jiaze and Chen, Kai and Dou, Qi},
  booktitle={2021 IEEE/RSJ International Conference on Intelligent Robots and Systems (IROS)},
  pages={4807--4814},
  year={2021},
  organization={IEEE}
}


@InProceedings{SGPA_2021_ICCV,
    author    = {Chen, Kai and Dou, Qi},
    title     = {SGPA: Structure-Guided Prior Adaptation for Category-Level 6D Object Pose Estimation},
    booktitle = {Proceedings of the IEEE/CVF International Conference on Computer Vision (ICCV)},
    month     = {October},
    year      = {2021},
    pages     = {2773-2782}
}

@article{UDA-COPE_2022_CVPR,
  author    = {Taeyeop Lee and
               Byeong{-}Uk Lee and
               Inkyu Shin and
               Jaesung Choe and
               Ukcheol Shin and
               In So Kweon and
               Kuk{-}Jin Yoon},
  title     = {{UDA-COPE:} Unsupervised Domain Adaptation for Category-level Object
               Pose Estimation},
  journal   = {CoRR},
  volume    = {abs/2111.12580},
  year      = {2021},
  url       = {https://arxiv.org/abs/2111.12580},
  eprinttype = {arXiv},
  eprint    = {2111.12580},
  timestamp = {Fri, 26 Nov 2021 13:48:43 +0100},
  biburl    = {https://dblp.org/rec/journals/corr/abs-2111-12580.bib},
  bibsource = {dblp computer science bibliography, https://dblp.org}
}

@article{CPSpp_2020,
  author    = {Fabian Manhardt and
               Manuel Nickel and
               Sven Meier and
               Luca Minciullo and
               Nassir Navab},
  title     = {{CPS:} Class-level 6D Pose and Shape Estimation From Monocular Images},
  journal   = {CoRR},
  volume    = {abs/2003.05848},
  year      = {2020},
  url       = {https://arxiv.org/abs/2003.05848},
  eprinttype = {arXiv},
  eprint    = {2003.05848},
  timestamp = {Tue, 17 Mar 2020 14:18:27 +0100},
  biburl    = {https://dblp.org/rec/journals/corr/abs-2003-05848.bib},
  bibsource = {dblp computer science bibliography, https://dblp.org}
}


@misc{ZebraPose_2022_CVPR,
  doi = {10.48550/ARXIV.2203.09418},
  
  url = {https://arxiv.org/abs/2203.09418},
  
  author = {Su, Yongzhi and Saleh, Mahdi and Fetzer, Torben and Rambach, Jason and Navab, Nassir and Busam, Benjamin and Stricker, Didier and Tombari, Federico},
  
  keywords = {Computer Vision and Pattern Recognition (cs.CV), FOS: Computer and information sciences, FOS: Computer and information sciences},
  
  title = {ZebraPose: Coarse to Fine Surface Encoding for 6DoF Object Pose Estimation},
  
  publisher = {arXiv},
  
  year = {2022},
  
  copyright = {arXiv.org perpetual, non-exclusive license}
}


@misc{Epro-PnP_2022_CVPR,
  doi = {10.48550/ARXIV.2203.13254},
  
  url = {https://arxiv.org/abs/2203.13254},
  
  author = {Chen, Hansheng and Wang, Pichao and Wang, Fan and Tian, Wei and Xiong, Lu and Li, Hao},
  
  keywords = {Computer Vision and Pattern Recognition (cs.CV), FOS: Computer and information sciences, FOS: Computer and information sciences},
  
  title = {EPro-PnP: Generalized End-to-End Probabilistic Perspective-n-Points for Monocular Object Pose Estimation},
  
  publisher = {arXiv},
  
  year = {2022},
  
  copyright = {arXiv.org perpetual, non-exclusive license}
}

@inproceedings{nerf_2020_ECCV_Mild,
  title={NeRF: Representing Scenes as Neural Radiance Fields for View Synthesis},
  author={Ben Mildenhall and Pratul P. Srinivasan and Matthew Tancik and Jonathan T. Barron and Ravi Ramamoorthi and Ren Ng},
  year={2020},
  booktitle={ECCV},
}

@article{instant_nerf_2022_mueller,
    title = {Instant Neural Graphics Primitives with a Multiresolution Hash Encoding},
    author = {Thomas M\"uller and Alex Evans and Christoph Schied and Alexander Keller},
    journal = {arXiv:2201.05989},
    year = {2022},
    month = jan
}

@inproceedings{GIRAFFE_2021_CVPR,
    title = {GIRAFFE: Representing Scenes as Compositional Generative Neural Feature Fields},
    author = {Niemeyer, Michael and Geiger, Andreas},
    booktitle = {Proc. IEEE Conf. on Computer Vision and Pattern Recognition (CVPR)},
    year = {2021}
}

@inproceedings{graf_Schwarz2020NEURIPS,
  title = {GRAF: Generative Radiance Fields for 3D-Aware Image Synthesis},
  author = {Schwarz, Katja and Liao, Yiyi and Niemeyer, Michael and Geiger, Andreas},
  booktitle = {Advances in Neural Information Processing Systems (NeurIPS)},
  year = {2020}
}

@InProceedings{SAR-Net_Lin_2022_CVPR,
    author    = {Lin, Haitao and Liu, Zichang and Cheang, Chilam and Fu, Yanwei and Guo, Guodong and Xue, Xiangyang},
    title     = {SAR-Net: Shape Alignment and Recovery Network for Category-Level 6D Object Pose and Size Estimation},
    booktitle = {Proceedings of the IEEE/CVF Conference on Computer Vision and Pattern Recognition (CVPR)},
    month     = {June},
    year      = {2022},
    pages     = {6707-6717}
}

@INPROCEEDINGS{3dgcn_lin_CVPR_2020,
  author={Lin, Zhi-Hao and Huang, Sheng-Yu and Wang, Yu-Chiang Frank},
  booktitle={2020 IEEE/CVF Conference on Computer Vision and Pattern Recognition (CVPR)}, 
  title={Convolution in the Cloud: Learning Deformable Kernels in 3D Graph Convolution Networks for Point Cloud Analysis}, 
  year={2020},
  volume={},
  number={},
  pages={1797-1806},
  doi={10.1109/CVPR42600.2020.00187}}

@inproceedings{zheng2022TPAE, 
    title={TP-AE: Temporally Primed 6D Object Pose Tracking with Auto-Encoders}, 
    author={Linfang, Zheng and Ales, Leonardis and Tze Ho, Elden, Tse and Nora, Horanyi and Hua, Chen and Wei, Zhang and Hyung Jin, Chang}, 
    booktitle={2022 IEEE International Conference on Robotics and Automation (ICRA)}, 
    year={2022} }


@article{edge_conv_TOG_2019,
  title={Dynamic Graph CNN for Learning on Point Clouds},
  author={Wang, Yue and Sun, Yongbin and Liu, Ziwei and Sarma, Sanjay E. and Bronstein, Michael M. and Solomon, Justin M.},
  journal={ACM Transactions on Graphics (TOG)},
  year={2019}
}

@inproceedings{inverse_gan_2021_CVPR,
    title = {Unsupervised 3D Shape Completion through GAN Inversion},
    author = {Zhang, Junzhe and Chen, Xinyi and Cai, Zhongang and Pan, Liang and Zhao, Haiyu 
    and Yi, Shuai and Yeo, Chai Kiat and Dai, Bo and Loy, Chen Change},
    booktitle = {CVPR},
    year = {2021}}

@article{wgan_gp_CoRR_2017,
  author    = {Ishaan Gulrajani and
               Faruk Ahmed and
               Mart{\'{\i}}n Arjovsky and
               Vincent Dumoulin and
               Aaron C. Courville},
  title     = {Improved Training of Wasserstein GANs},
  journal   = {CoRR},
  volume    = {abs/1704.00028},
  year      = {2017},
  url       = {http://arxiv.org/abs/1704.00028},
  eprinttype = {arXiv},
  eprint    = {1704.00028},
  timestamp = {Mon, 13 Aug 2018 16:47:43 +0200},
  biburl    = {https://dblp.org/rec/journals/corr/GulrajaniAADC17.bib},
  bibsource = {dblp computer science bibliography, https://dblp.org}
}


@InProceedings{PhoCal_Wang_2022_CVPR,
    author    = {Wang, Pengyuan and Jung, HyunJun and Li, Yitong and Shen, Siyuan and Srikanth, Rahul Parthasarathy and Garattoni, Lorenzo and Meier, Sven and Navab, Nassir and Busam, Benjamin},
    title     = {PhoCaL: A Multi-Modal Dataset for Category-Level Object Pose Estimation With Photometrically Challenging Objects},
    booktitle = {Proceedings of the IEEE/CVF Conference on Computer Vision and Pattern Recognition (CVPR)},
    month     = {June},
    year      = {2022},
    pages     = {21222-21231}
}


@INPROCEEDINGS{BundleTrack_IROS_2021,  author={Wen, Bowen and Bekris, Kostas},  booktitle={2021 IEEE/RSJ International Conference on Intelligent Robots and Systems (IROS)},   title={BundleTrack: 6D Pose Tracking for Novel Objects without Instance or Category-Level 3D Models},   year={2021},  volume={},  number={},  pages={8067-8074},  doi={10.1109/IROS51168.2021.9635991}}

@InProceedings{template-pose_Nguyen_2022_CVPR,
    author    = {Nguyen, Van Nguyen and Hu, Yinlin and Xiao, Yang and Salzmann, Mathieu and Lepetit, Vincent},
    title     = {Templates for 3D Object Pose Estimation Revisited: Generalization to New Objects and Robustness to Occlusions},
    booktitle = {Proceedings of the IEEE/CVF Conference on Computer Vision and Pattern Recognition (CVPR)},
    month     = {June},
    year      = {2022},
    pages     = {6771-6780}
}

@article{SurfEmb_2022_CVPR,
  author    = {Rasmus Laurvig Haugaard and
               Anders Glent Buch},
  title     = {SurfEmb: Dense and Continuous Correspondence Distributions for Object
               Pose Estimation with Learnt Surface Embeddings},
  journal   = {CoRR},
  volume    = {abs/2111.13489},
  year      = {2021},
  url       = {https://arxiv.org/abs/2111.13489},
  eprinttype = {arXiv},
  eprint    = {2111.13489},
  timestamp = {Wed, 01 Dec 2021 15:16:43 +0100},
  biburl    = {https://dblp.org/rec/journals/corr/abs-2111-13489.bib},
  bibsource = {dblp computer science bibliography, https://dblp.org}
}

@InProceedings{StructuredLS_Cai_2022_CVPR,
    author    = {Cai, Yingjie and Lin, Kwan-Yee and Zhang, Chao and Wang, Qiang and Wang, Xiaogang and Li, Hongsheng},
    title     = {Learning a Structured Latent Space for Unsupervised Point Cloud Completion},
    booktitle = {Proceedings of the IEEE/CVF Conference on Computer Vision and Pattern Recognition (CVPR)},
    month     = {June},
    year      = {2022},
    pages     = {5543-5553}
}

@article{PCN,
  author    = {Wentao Yuan and
               Tejas Khot and
               David Held and
               Christoph Mertz and
               Martial Hebert},
  title     = {{PCN:} Point Completion Network},
  journal   = {CoRR},
  volume    = {abs/1808.00671},
  year      = {2018},
  url       = {http://arxiv.org/abs/1808.00671},
  eprinttype = {arXiv},
  eprint    = {1808.00671},
  timestamp = {Thu, 14 Oct 2021 09:15:25 +0200},
  biburl    = {https://dblp.org/rec/journals/corr/abs-1808-00671.bib},
  bibsource = {dblp computer science bibliography, https://dblp.org}
}

@article{GRnet_2020_ECCV,
  author    = {Haozhe Xie and
               Hongxun Yao and
               Shangchen Zhou and
               Jiageng Mao and
               Shengping Zhang and
               Wenxiu Sun},
  title     = {GRNet: Gridding Residual Network for Dense Point Cloud Completion},
  journal   = {CoRR},
  volume    = {abs/2006.03761},
  year      = {2020},
  url       = {https://arxiv.org/abs/2006.03761},
  eprinttype = {arXiv},
  eprint    = {2006.03761},
  timestamp = {Fri, 12 Jun 2020 14:02:57 +0200},
  biburl    = {https://dblp.org/rec/journals/corr/abs-2006-03761.bib},
  bibsource = {dblp computer science bibliography, https://dblp.org}
}

@article{Detailed_PC_Completion_2020_ECCV,
  author    = {Wenxiao Zhang and
               Qingan Yan and
               Chunxia Xiao},
  title     = {Detail Preserved Point Cloud Completion via Separated Feature Aggregation},
  journal   = {CoRR},
  volume    = {abs/2007.02374},
  year      = {2020},
  url       = {https://arxiv.org/abs/2007.02374},
  eprinttype = {arXiv},
  eprint    = {2007.02374},
  timestamp = {Fri, 17 Jul 2020 15:39:46 +0200},
  biburl    = {https://dblp.org/rec/journals/corr/abs-2007-02374.bib},
  bibsource = {dblp computer science bibliography, https://dblp.org}
}

@inproceedings{cycle4completion_CVPR_2021,
  title={Cycle4Completion: Unpaired Point Cloud Completion using Cycle Transformation with Missing Region Coding},
  author={Wen, Xin and Han, Zhizhong and Cao, Yan-Pei and Wan, Pengfei and Zheng, Wen and Liu, Yu-Shen},
  booktitle={Proceedings of the IEEE Conference on Computer Vision and Pattern Recognition (CVPR)},
  year={2021}
}

@inproceedings{shapeInversion_2021_CVPR,
    title = {Unsupervised 3D Shape Completion through GAN Inversion},
    author = {Zhang, Junzhe and Chen, Xinyi and Cai, Zhongang and Pan, Liang and Zhao, Haiyu 
    and Yi, Shuai and Yeo, Chai Kiat and Dai, Bo and Loy, Chen Change},
    booktitle = {CVPR},
    year = {2021}}

@InProceedings{PVN3D_CVPR_2019,
author = {He, Yisheng and Sun, Wei and Huang, Haibin and Liu, Jianran and Fan, Haoqiang and Sun, Jian},
title = {PVN3D: A Deep Point-Wise 3D Keypoints Voting Network for 6DoF Pose Estimation},
booktitle = {IEEE/CVF Conference on Computer Vision and Pattern Recognition (CVPR)},
month = {June},
year = {2020}
}

 @InProceedings{CASS_2020_CVPR,
author = {Chen, Dengsheng and Li, Jun and Wang, Zheng and Xu, Kai},
title = {Learning Canonical Shape Space for Category-Level 6D Object Pose and Size Estimation},
booktitle = {Proceedings of the IEEE/CVF Conference on Computer Vision and Pattern Recognition (CVPR)},
month = {June},
year = {2020}
}

@InProceedings{FSNET_2021_CVPR,
    author    = {Chen, Wei and Jia, Xi and Chang, Hyung Jin and Duan, Jinming and Shen, Linlin and Leonardis, Ales},
    title     = {FS-Net: Fast Shape-Based Network for Category-Level 6D Object Pose Estimation With Decoupled Rotation Mechanism},
    booktitle = {Proceedings of the IEEE/CVF Conference on Computer Vision and Pattern Recognition (CVPR)},
    month     = {June},
    year      = {2021},
    pages     = {1581-1590}
}

@InProceedings{FSNET_2021_CVPR_reb,
    author    = {Chen et al.},
    title     = {{FS-Net}: Fast Shape-Based Network for Category-Level 6D Object Pose Estimation With Decoupled Rotation Mechanism},
    booktitle = {CVPR},
    month     = {June},
    year      = {2021}
}

@article{CAPTRA_2021,
	title={CAPTRA: CAtegory-level Pose Tracking for Rigid and Articulated Objects from Point Clouds},
	author={Weng, Yijia and Wang, He and Zhou, Qiang and Qin, Yuzhe and Duan, Yueqi and Fan, Qingnan and Chen, Baoquan and Su, Hao and Guibas, Leonidas J},
	journal={arXiv preprint arXiv:2104.03437},
	year={2021}
	}

@InProceedings{Tian_ShapePrior_2020_ECCV,
  author = {Tian, Meng and Ang Jr, Marcelo H and Lee, Gim Hee},
  title = {Shape Prior Deformation for Categorical 6D Object Pose and Size Estimation},
  booktitle = {Proceedings of the European Conference on Computer Vision (ECCV)},
  month = {August},
  year = {2020}
}


@InProceedings{liu_2022_catre,
  title     = {{CATRE:} Iterative Point Clouds Alignment for Category-level Object Pose Refinement},
  author    = {Liu, Xingyu and Wang, Gu and Li, Yi and Ji, Xiangyang},
  booktitle = {European Conference on Computer Vision (ECCV)},
  month     = {October},
  year      = {2022}
}

@unknown{SSCO-use-3dgcn,
author = {He, Yisheng and Fan, Haoqiang and Haibin, Huang and Chen, Qifeng and Sun, Jian},
year = {2022},
month = {03},
pages = {},
title = {Towards Self-Supervised Category-Level Object Pose and Size Estimation}
}

@unknown{SSP-Pose_arxiv,
author = {Zhang, Ruida and Di, Yan and Manhardt, Fabian and Tombari, Federico and Ji, Xiangyang},
year = {2022},
month = {08},
pages = {},
title = {SSP-Pose: Symmetry-Aware Shape Prior Deformation for Direct Category-Level Object Pose Estimation},
doi = {10.48550/arXiv.2208.06661}
}

@unknown{RBP-Pose_arxiv,
author = {Zhang, Ruida and Di, Yan and Lou, Zhiqiang and Manhardt, Fabian and Navab, Nassir and Tombari, Federico and Ji, Xiangyang},
year = {2022},
month = {07},
pages = {},
title = {RBP-Pose: Residual Bounding Box Projection for Category-Level Pose Estimation},
doi = {10.48550/arXiv.2208.00237}
}

@misc{RBP-Pose_ECCV_2022,
  doi = {10.48550/ARXIV.2208.00237},
  
  url = {https://arxiv.org/abs/2208.00237},
  
  author = {Zhang, Ruida and Di, Yan and Lou, Zhiqiang and Manhardt, Fabian and Tombari, Federico and Ji, Xiangyang},
  
  keywords = {Computer Vision and Pattern Recognition (cs.CV), FOS: Computer and information sciences, FOS: Computer and information sciences},
  
  title = {RBP-Pose: Residual Bounding Box Projection for Category-Level Pose Estimation},
  
  publisher = {arXiv},
  
  year = {2022},
  
  copyright = {Creative Commons Attribution Non Commercial Share Alike 4.0 International}
}

@misc{SSP-Pose_IROS_22,
  doi = {10.48550/ARXIV.2208.06661},
  
  url = {https://arxiv.org/abs/2208.06661},
  
  author = {Zhang, Ruida and Di, Yan and Manhardt, Fabian and Tombari, Federico and Ji, Xiangyang},
  
  keywords = {Computer Vision and Pattern Recognition (cs.CV), FOS: Computer and information sciences, FOS: Computer and information sciences},
  
  title = {SSP-Pose: Symmetry-Aware Shape Prior Deformation for Direct Category-Level Object Pose Estimation},
  
  publisher = {arXiv},
  
  year = {2022},
  
  copyright = {Creative Commons Attribution Non Commercial Share Alike 4.0 International}
}

@INPROCEEDINGS{augmented_reality_application_2021,

  author={Su, Yongzhi and Rambach, Jason and Minaskan, Nareg and Lesur, Paul and Pagani, Alain and Stricker, Didier},

  booktitle={2019 IEEE International Symposium on Mixed and Augmented Reality Adjunct (ISMAR-Adjunct)}, 

  title={Deep Multi-state Object Pose Estimation for Augmented Reality Assembly}, 

  year={2019},

  volume={},

  number={},

  pages={222-227},

  doi={10.1109/ISMAR-Adjunct.2019.00-42}}

@inproceedings{autonomous_driving_application_2017,
author = {Kothari, Nikunj and Gupta, Misha and Vachhani, Leena and Arya, Hemendra},
year = {2017},
month = {01},
pages = {424-431},
title = {Pose estimation for an autonomous vehicle using monocular vision},
doi = {10.1109/INDIANCC.2017.7846512}
}

@misc{Self-DPDN_ECCV_2022,
  doi = {10.48550/ARXIV.2207.05444},
  
  url = {https://arxiv.org/abs/2207.05444},
  
  author = {Lin, Jiehong and Wei, Zewei and Ding, Changxing and Jia, Kui},
  
  keywords = {Computer Vision and Pattern Recognition (cs.CV), FOS: Computer and information sciences, FOS: Computer and information sciences},
  
  title = {Category-Level 6D Object Pose and Size Estimation using Self-Supervised Deep Prior Deformation Networks},
  
  publisher = {arXiv},
  
  year = {2022},
  
  copyright = {arXiv.org perpetual, non-exclusive license}
}

@inproceedings{ShaPO_ECCV_2022,
  title={ShAPO: Implicit Representations for Multi Object Shape Appearance and Pose Optimization},
  author={Muhammad Zubair Irshad and Sergey Zakharov and Rares Ambrus and Thomas Kollar and Zsolt Kira and Adrien Gaidon},
  journal={European Conference on Computer Vision (ECCV)},
  year={2022},
  url={https://arxiv.org/abs/2207.13691},
}

@misc{TransNet_ECCV_2022,
  doi = {10.48550/ARXIV.2208.10002},
  
  url = {https://arxiv.org/abs/2208.10002},
  
  author = {Zhang, Huijie and Opipari, Anthony and Chen, Xiaotong and Zhu, Jiyue and Yu, Zeren and Jenkins, Odest Chadwicke},
  
  keywords = {Computer Vision and Pattern Recognition (cs.CV), Robotics (cs.RO), FOS: Computer and information sciences, FOS: Computer and information sciences},
  
  title = {TransNet: Category-Level Transparent Object Pose Estimation},
  
  publisher = {arXiv},
  
  year = {2022},
  
  copyright = {Creative Commons Attribution 4.0 International}
}

@misc{Temp6D_CVPR_22,
  doi = {10.48550/ARXIV.2203.17234},
  
  url = {https://arxiv.org/abs/2203.17234},
  
  author = {Nguyen, Van Nguyen and Hu, Yinlin and Xiao, Yang and Salzmann, Mathieu and Lepetit, Vincent},
  
  keywords = {Computer Vision and Pattern Recognition (cs.CV), FOS: Computer and information sciences, FOS: Computer and information sciences},
  
  title = {Templates for 3D Object Pose Estimation Revisited: Generalization to New Objects and Robustness to Occlusions},
  
  publisher = {arXiv},
  
  year = {2022},
  
  copyright = {arXiv.org perpetual, non-exclusive license}
}

@misc{MP-Encoder_CVPR_2020,
  doi = {10.48550/ARXIV.1908.00151},
  
  url = {https://arxiv.org/abs/1908.00151},
  
  author = {Sundermeyer, Martin and Durner, Maximilian and Puang, En Yen and Marton, Zoltan-Csaba and Vaskevicius, Narunas and Arras, Kai O. and Triebel, Rudolph},
  
  keywords = {Computer Vision and Pattern Recognition (cs.CV), Machine Learning (stat.ML), FOS: Computer and information sciences, FOS: Computer and information sciences},
  
  title = {Multi-path Learning for Object Pose Estimation Across Domains},
  
  publisher = {arXiv},
  
  year = {2019},
  
  copyright = {arXiv.org perpetual, non-exclusive license}
}

@incollection{Hinterstoisser_2016_PPF,
	doi = {10.1007/978-3-319-46487-9_51},
  
	url = {https://doi.org/10.1007%2F978-3-319-46487-9_51},
  
	year = 2016,
	publisher = {Springer International Publishing},
  
	pages = {834--848},
  
	author = {Stefan Hinterstoisser and Vincent Lepetit and Naresh Rajkumar and Kurt Konolige},
  
	title = {Going Further with Point Pair Features},
  
	booktitle = {Computer Vision {\textendash} {ECCV} 2016}
}
}

@misc{Vidal_matching_PPF_2018,
  doi = {10.48550/ARXIV.1802.08516},
  
  url = {https://arxiv.org/abs/1802.08516},
  
  author = {Vidal, Joel and Lin, Chyi-Yeu and Martí, Robert},
  
  keywords = {Computer Vision and Pattern Recognition (cs.CV), FOS: Computer and information sciences, FOS: Computer and information sciences},
  
  title = {6D Pose Estimation using an Improved Method based on Point Pair Features},
  
  publisher = {arXiv},
  
  year = {2018},
  
  copyright = {arXiv.org perpetual, non-exclusive license}
}


@misc{Tremblay_2018_Bbox_Corners,
  doi = {10.48550/ARXIV.1809.10790},
  
  url = {https://arxiv.org/abs/1809.10790},
  
  author = {Tremblay, Jonathan and To, Thang and Sundaralingam, Balakumar and Xiang, Yu and Fox, Dieter and Birchfield, Stan},
  
  keywords = {Robotics (cs.RO), FOS: Computer and information sciences, FOS: Computer and information sciences},
  
  title = {Deep Object Pose Estimation for Semantic Robotic Grasping of Household Objects},
  
  publisher = {arXiv},
  
  year = {2018},
  
  copyright = {arXiv.org perpetual, non-exclusive license}
}

@misc{Manhart_deep_model_regression,
  doi = {10.48550/ARXIV.1810.03065},
  
  url = {https://arxiv.org/abs/1810.03065},
  
  author = {Manhardt, Fabian and Kehl, Wadim and Navab, Nassir and Tombari, Federico},
  
  keywords = {Computer Vision and Pattern Recognition (cs.CV), FOS: Computer and information sciences, FOS: Computer and information sciences},
  
  title = {Deep Model-Based 6D Pose Refinement in RGB},
  
  publisher = {arXiv},
  
  year = {2018},
  
  copyright = {arXiv.org perpetual, non-exclusive license}
}

@misc{ranger_optimizer_1_ICLA_2019,
  doi = {10.48550/ARXIV.1908.03265},
  
  url = {https://arxiv.org/abs/1908.03265},
  
  author = {Liu, Liyuan and Jiang, Haoming and He, Pengcheng and Chen, Weizhu and Liu, Xiaodong and Gao, Jianfeng and Han, Jiawei},
  
  keywords = {Machine Learning (cs.LG), Computation and Language (cs.CL), Machine Learning (stat.ML), FOS: Computer and information sciences, FOS: Computer and information sciences},
  
  title = {On the Variance of the Adaptive Learning Rate and Beyond},
  
  publisher = {arXiv},
  
  year = {2019},
  
  copyright = {arXiv.org perpetual, non-exclusive license}
}

@misc{Ranger_optimizer_2_ECCV_2020,
  doi = {10.48550/ARXIV.2004.01461},
  
  url = {https://arxiv.org/abs/2004.01461},
  
  author = {Yong, Hongwei and Huang, Jianqiang and Hua, Xiansheng and Zhang, Lei},
  
  keywords = {Computer Vision and Pattern Recognition (cs.CV), FOS: Computer and information sciences, FOS: Computer and information sciences},
  
  title = {Gradient Centralization: A New Optimization Technique for Deep Neural Networks},
  
  publisher = {arXiv},
  
  year = {2020},
  
  copyright = {arXiv.org perpetual, non-exclusive license}
}

@misc{Ranger_optimizer_3_2019_NIPS,
  doi = {10.48550/ARXIV.1907.08610},
  
  url = {https://arxiv.org/abs/1907.08610},
  
  author = {Zhang, Michael R. and Lucas, James and Hinton, Geoffrey and Ba, Jimmy},
  
  keywords = {Machine Learning (cs.LG), Neural and Evolutionary Computing (cs.NE), Machine Learning (stat.ML), FOS: Computer and information sciences, FOS: Computer and information sciences},
  
  title = {Lookahead Optimizer: k steps forward, 1 step back},
  
  publisher = {arXiv},
  
  year = {2019},
  
  copyright = {arXiv.org perpetual, non-exclusive license}
}

@InProceedings{OSOP_2022_CVPR,
    author    = {Shugurov, Ivan and Li, Fu and Busam, Benjamin and Ilic, Slobodan},
    title     = {OSOP: A Multi-Stage One Shot Object Pose Estimation Framework},
    booktitle = {Proceedings of the IEEE/CVF Conference on Computer Vision and Pattern Recognition (CVPR)},
    month     = {June},
    year      = {2022},
    pages     = {6835-6844}
}


@InProceedings{OVE6D_2022_CVPR,
    author    = {Cai, Dingding and Heikkil\"a, Janne and Rahtu, Esa},
    title     = {OVE6D: Object Viewpoint Encoding for Depth-Based 6D Object Pose Estimation},
    booktitle = {Proceedings of the IEEE/CVF Conference on Computer Vision and Pattern Recognition (CVPR)},
    month     = {June},
    year      = {2022},
    pages     = {6803-6813}
}

@InProceedings{SLAM6D_2022_CVPR,
    author    = {Merrill, Nathaniel and Guo, Yuliang and Zuo, Xingxing and Huang, Xinyu and Leutenegger, Stefan and Peng, Xi and Ren, Liu and Huang, Guoquan},
    title     = {Symmetry and Uncertainty-Aware Object SLAM for 6DoF Object Pose Estimation},
    booktitle = {Proceedings of the IEEE/CVF Conference on Computer Vision and Pattern Recognition (CVPR)},
    month     = {June},
    year      = {2022},
    pages     = {14901-14910}
}

@InProceedings{RNNPose_2022_CVPR,
    author    = {Xu, Yan and Lin, Kwan-Yee and Zhang, Guofeng and Wang, Xiaogang and Li, Hongsheng},
    title     = {RNNPose: Recurrent 6-DoF Object Pose Refinement With Robust Correspondence Field Estimation and Pose Optimization},
    booktitle = {Proceedings of the IEEE/CVF Conference on Computer Vision and Pattern Recognition (CVPR)},
    month     = {June},
    year      = {2022},
    pages     = {14880-14890}
}

@article{6D_pack_2020_ICRA,
  title={6-PACK: Category-level 6D Pose Tracker with Anchor-Based Keypoints},
  author={Wang, Chen and Mart{\'\i}n-Mart{\'\i}n, Roberto and Xu, Danfei and Lv, Jun and Lu, Cewu and Fei-Fei, Li and Savarese, Silvio and Zhu, Yuke},
  booktitle={International Conference on Robotics and Automation (ICRA)},
  year={2020}
}

@InProceedings{ES6D_2022_CVPR,
    author    = {Mo, Ningkai and Gan, Wanshui and Yokoya, Naoto and Chen, Shifeng},
    title     = {ES6D: A Computation Efficient and Symmetry-Aware 6D Pose Regression Framework},
    booktitle = {Proceedings of the IEEE/CVF Conference on Computer Vision and Pattern Recognition (CVPR)},
    month     = {June},
    year      = {2022},
    pages     = {6718-6727}
}

@inproceedings{SD-MaskRCNN_ICRA_2019,
  title={Segmenting Unknown 3D Objects from Real Depth Images using Mask R-CNN Trained on Synthetic Data},
  author={Danielczuk, Michael and Matl, Matthew and Gupta, Saurabh and Li, Andrew and Lee, Andrew and Mahler, Jeffrey and Goldberg, Ken},
  booktitle={Proc. IEEE Int. Conf. Robotics and Automation (ICRA)},
  year={2019}
}

@article{SS-conv,
title={Sparse Steerable Convolutions: An Efficient Learning of SE (3)-Equivariant Features for Estimation and Tracking of Object Poses in 3D Space},
author={Lin, Jiehong and Li, Hongyang and Chen, Ke and Lu, Jiangbo and Jia, Kui},
journal={Advances in Neural Information Processing Systems},
volume={34},
year={2021}
}
